On Semantic Generalizations of the Bernays-Sch\"onfinkel-Ramsey Class with Finite or Co-finite Spectra

Motivated by model-theoretic properties of the BSR class, we present a family of semantic classes of FO formulae with finite or co-finite spectra over a relational vocabulary \Sigma. A class in this family is denoted EBS_\Sigma(\sigma), where \sigma is a subset of \Sigma. Formulae in EBS_\Sigma(\sigma) are preserved under substructures modulo a bounded core and modulo re-interpretation of predicates outside \sigma. We study properties of the family EBS_\Sigma = {EBS_\Sigma(\sigma) | \sigma \subseteq \Sigma}, e.g. classes in EBS_\Sigma are spectrally indistinguishable, EBS_\Sigma(\Sigma) is semantically equivalent to BSR over \Sigma, and EBS_\Sigma(\emptyset) is the set of all FO formulae over \Sigma with finite or co-finite spectra. Furthermore, (EBS_\Sigma, \subseteq) forms a lattice isomorphic to the powerset lattice (\wp({\Sigma}), \subseteq). This gives a natural semantic generalization of BSR as ascending chains in (EBS_\Sigma, \subseteq). Many well-known FO classes are semantically subsumed by EBS_\Sigma(\Sigma) or EBS_\Sigma(\emptyset). Our study provides alternative proofs of interesting results like the Lo\'s-Tarski Theorem and the semantic subsumption of the L\"owenheim class with equality by BSR. We also present a syntactic sub-class of EBS_\Sigma(\sigma) called EDP_\Sigma(\sigma) and give an expression for the size of the bounded cores of models of EDP_\Sigma(\sigma) formulae. We show that the EDP_\Sigma(\sigma) classes also form a lattice structure. Finally, we study some closure properties and applications of the classes presented.

==> EBS_equals_BSR.tex <==
\section{$\ebsS{\Sigma}$ as a semantic characterization of
  $\bsrS$}\label{section:ebs_and_bsr}
\begin{theorem}\label{thm:lowest_EBS_equals_BSR}
A sentence $\phi \in \ebsS{\Sigma}$ iff there exists a
sentence $\psi \in \bsrS$ equivalent to $\phi$.
\end{theorem}

\ti{Proof}:

Given a {\bsrS} sentence $\psi$, from the proof of the small model
property of $\bsrS$ as given in ~\cite{BGG}, it can be seen that $\psi
\in \ebsSS$ with bound $\mc{B}$ being atmost the number of existential
quantifiers of $\psi$. Then since \ebsSS is a semantic clss, if $\psi$
is equivalent to $\phi$, then $\phi$ also belongs to \ebsSS.


Consider $\phi \in \ebsS{\Sigma}$ in PCNF. W.l.o.g. let
\[
\phi = \forall \tbf{z}_0 \exists v_1 \forall \tbf{z}_1 \exists v_2 
\forall \tbf{z}_2 \ldots \exists v_r \forall \tbf{z}_r 
\xi(\tbf{z}, v_1 \ldots, v_r)
\]
where $\tbf{z} = (\tbf{z}_0, \ldots, \tbf{z}_r)$ and $\xi$ is
quantifier-free. Let $S_{\tbf{z}}$ be the set of variables of
$\tbf{z}$. Introduce fresh variables $x_1, \ldots, x_{\mc{B}}$ where
$\mc{B}$ is the bound for $\phi$ and let $\mc{V} = \{x_1, \ldots,
x_{\mc{B}}\} \cup S_{\tbf{z}}$. Consider $\psi$ as below.\\

\begin{tabular}{lll}
$\psi$ & = & $\exists x_1 \ldots \exists x_{\mc{B}} \forall \tbf{z}_0
\forall \tbf{z}_1 \ldots \forall \tbf{z}_r ~(\chi)~$ where\\
$\chi$ & = & $(\bigvee_{u_1 \in \mc{V}} \ldots \bigvee_{u_r \in \mc{V}} \xi
(\tbf{z}, v_1 \mapsto u_1, \ldots, v_r \mapsto u_r))$\\
\end{tabular}

Here $\xi (\tbf{z}, v_1 \mapsto u_1, \ldots, v_r \mapsto u_r)$ is the
formula obtained by replacing every occurence of $v_i$ in $\xi$ by
$u_i$.

If $M \models \phi$ and $|\mc{U}_M| \leq \mc{B}$, then assign values
to $x_1 \ldots x_{\mc{B}}$ such that each $a \in \mc{U}_{M}$ is
assigned to some $x_i$. Consider an instantiation $\mc{Z}$ of \tbf{z}
from $\mc{U}_M$. Since $M \models \phi$, there exist values $d_1,
\ldots, d_r$ for $v_1, \ldots, v_r$ such that $M \models \xi(\mc{Z},
d_1, \ldots, d_r)$. Each $d_i$ is the value assigned to some $u_i \in
\{x_1, \ldots, x_{\mc{B}}\}$. Then $M \models \xi (\mc{Z}, v_1
\mapsto u_1, \ldots, v_r \mapsto u_r)$ and so $M \models \chi$. Since
$\mc{Z}$ was arbitrary, $M \models \psi$.

If $M \models \phi$ and $|\mc{U}_M| \geq \mc{B}$, then there exists
$M_1 \subseteq M$ satisfying the $\ebsS{\Sigma}$
conditions. Assign values to $x_1 \ldots x_{\mc{B}}$ s.t. each $x_i$
is assigned some $a \in \mc{U}_{M_1}$ and each $a \in \mc{U}_{M_1}$ is
assigned to some $x_j$. Consider an instantiation $\mc{Z}$ of \tbf{z}.
Let the set of elements of $\mc{Z}$ be $\mc{T}$. Then consider the
substructure $M_2$ of $M$ generated by $\mc{U}_{M_1} \cup ~\mc{T}$.
Since $M_1 \subseteq M_2 \subseteq M$, $M_2 \models \phi$.  Then there
exist values $d_1, \ldots, d_r$ for $v_1, \ldots, v_r$ such that $M_2
\models \xi(\mc{Z}, d_1, \ldots, d_r)$. Observe that since $M_2
\subseteq M$, $M \models \xi(\mc{Z}, d_1, \ldots, d_r)$.  Now since
$d_i \in \mc{U}_{M_1} \cup ~\mc{T}$, it is the value assigned to some
$u_i \in \mc{V}$. Then since $M \models \xi(\mc{Z}, d_1, \ldots,
d_r)$, $M \models \xi(\mc{Z}, v_1 \mapsto u_1, \ldots, v_r \mapsto
u_r)$ and so $M \models \chi$. Since $\mc{Z}$ was arbitrary, $M
\models \psi$.\\

Now suppose $M \models \psi$. Then there exists a set of values $S
\subseteq \mc{U}_M$ such that the $x_i$'s in $\psi$ get their values
from this set and for all instantiations from $\mc{U}_M$ of \tbf{z},
$M \models \chi$. Then consider the instantiation $\mc{Z}$ of
\tbf{z}. Since $M \models \chi$ for $\mc{Z}$, there exists some
disjunct $\xi (\mc{Z}, v_1 \mapsto u_1; \ldots; v_r \mapsto u_r)$
which is $\mathsf{True}$ in $M$. Now $u_i \in \mc{V}$ and hence is
either some $x_j$ or a universal variable $z$. Then if $u_i$ is $x_j$,
let $d_i$ be the value (from $S$) assigned to $x_j$.  If $u_i$ is the
variable $z$, let $d_i$ be the value assigned to $z$ in $\mc{Z}$. Then
$M \models \xi (\mc{Z}, d_1 \ldots, d_r)$. Then for the instantiation
$\mc{Z}$, choosing $v_i = d_i$, we see that the matrix of $\phi$
becomes $\mathsf{True}$ in $M$. Doing likewise for all instantiations
of $\tbf{z}$, we conclude that $M \models \phi$.


From the above then, $M \models \phi \leftrightarrow M \models \psi$
i.e. $\phi$ is equivalent to $\psi$, the latter being a sentence in
$\bsrS$. \epf\\



\underline{\tbf{Some consequences of Theorem
  \ref{thm:lowest_EBS_equals_BSR}}}

\begin{enumerate}
\item \ti{Lo\'s-Tarski Theorem as a special case:}~Consider the class
  of {\FOS} sentences $\phi$ which are preserved under
  substructures. Then we can see that $\phi \in
  \ebsS{\Sigma}$ with $\mc{B} = 0$. Then from the proof
  of the Theorem \ref{thm:lowest_EBS_equals_BSR}, we can see that
  $\phi$ is equivalent to a $\bsrS$ sentence $\psi$ where
  the number of existential quantifiers is 0. In other words $\phi$ is
  equivalent to a $\forall^*$ sentence. The converse, namely, that a
  $\forall^*$ sentence is closed under substructures is well-known. We
  thus get the Lo\'s-Tarski Theorem as a special case of Theorem
  \ref{thm:lowest_EBS_equals_BSR}. The proof of Theorem
  \ref{thm:lowest_EBS_equals_BSR} serves as an alternate proof of the
  Lo\'s-Tarski Theorem.

  The $\ebsS{\Sigma}$ property can be viewed as preservation under
  substructures \ti{modulo a bounded `core'} i.e. all substructures of
  a model which contain the core of the model are also models. The
  $\exists^*$ quantifiers in the equivalent $\bsrS$ formula of an
  $\ebsS{\Sigma}$ formula can be seen to assert the existence of a
  bounded extensible core.

\item \ti{$\bsrS$ semantically subsumes other classes:} Theorem
  \ref{thm:lowest_EBS_equals_BSR} helps to show right away that some
  classes of {\FOS} formulae are semantically contained in
  $\bsrS$. The L\"owenheim class is the class of all {\FOS} sentences
  over $\Sigma$, without equality where $\Sigma$ contains only unary
  predicates. The L\"owenheim class with equality - denoted
  $\tbf{L}_{\Sigma}$ - is the class of all {\FOS} sentences over
  $\Sigma$, possibly containing equality where $\Sigma$ contains only
  unary predicates (Whenever we will talk about just the L\"ownheim
  class, we will refer to it as `$\tbf{L}_{\Sigma}$ without
  equality').  By an Ehrenfeucht-Fra\"iss\'e game argument (see
  ~\cite{BGG}, pp. 259), one can show that if $\phi \in
  \tbf{L}_{\Sigma}$, then $\phi \in \ebsS{\Sigma}$ with the bound
  $\mc{B} = q \cdot 2^m$ where $q$ is the length of the quantifier
  prefix of $\phi$ and $m$ is the number of unary predicates ($m =
  |\Sigma|$). By theorem \ref{thm:lowest_EBS_equals_BSR}, we
  immediately know that for $\phi$, there is an equivalent $\bsrS$
  sentence $\psi$ whose number of existential quantifiers is
  $\mc{B}$. Since $\Sigma$ contains only unary predicates, this shows
  us that $\tbf{L}_{\Sigma}$ is semantically the same as the $\bsrS$
  class, the latter being a proper syntactic subset of the former.

  Other known classes which can be seen to be subsumed semantically by
  $\bsrS$ include $\FOS[1]$ and $\FOS[1]$ with counting which are
  respectively the class of {\FOS} sentences having only one variable
  and the class of {\FOS} sentences with counting having only one
  variable. These are contained inside $\tbf{L}_{\Sigma}$ and hence
  are semantically within $\bsrS$.



\item \ti{Translation from $\ebsS{\Sigma}$ to
  $\bsrS$:} The proof not only shows us that for a
  sentence $\phi \in \ebsS{\Sigma}$, there exists an
  equivalent $\bsrS$ sentence, but also gives us the
  sentence ($\psi$ in the proof).  It gives a uniform translation
  scheme from the whole of $\ebsS{\Sigma}$ to
  $\bsrS$. As for the size of $\psi$, the number of
  $\exists$ variables is $\mc{B}$, the number of $\forall$ variables
  is atmost $k + 1$ where $k$ is the number of $\forall$ variables in
  $\phi$ and the size of the matrix is $O((\mc{B} + k + 1)^r \cdot
  |\xi|)$ where $|\xi|$ is the length of $\xi$ and where $r$ (number
  of existential quantifiers) and $\xi$ are as in the proof.

\item \ti{Optimal translation:} The proof also shows us that for a
  sentence $\phi \in \ebsS{\Sigma}$ whose bound is
  $\mc{B}$, there cannot exist an equivalent $\bsrS$
  sentence with $\mc{B}' ~ \exists$ quantifiers where $\mc{B}' <
  \mc{B}$.  Otherwise, we would violate the minimality of $\mc{B}$.

\item \ti{Finding the bound $\mc{B}$:} $\ebsS{\Sigma}$ is exactly the
  class of all those sentences which are equivalent to formulae in
  $\bsrS$.  This syntactic characterization of $\ebsS{\Sigma}$ as
  $\bsrS$, the latter being a syntactic class for which membership is
  decidable, shows us that the membership problem for $\ebsS{\Sigma}$
  is recursively enumerable (We show later that the membership problem
  for $\ebsS{\Sigma}$ is undecidable though in general). Suppose we
  knew that $\phi$ belongs to $\ebsS{\Sigma}$, but did not know the
  bound $\mc{B}$ for $\phi$.  A naive approach would be to try to
  prove equivalence of $\phi$ with each {\bsrS} formula with $k$
  $\exists$ quantifiers, for increasing values of $k$.  The above
  proof however shows that for each $k$, it is sufficient to construct
  \ti{exactly one} $\bsrS$ formula with which the equivalence of
  $\phi$ needs to be checked. Following is the procedure of finding
  $\mc{B}$ in detail:

  For each $\mc{B} \geq 0$, we construct the formula $\psi$ as shown
  in the proof. Call this formula $\psi_{\mc{B}}$. We then construct
  the formula $\Xi_{\mc{B}} = (\phi \leftrightarrow
  \psi_{\mc{B}})$. We then interleave the procedures which check for
  the validity of $\Xi_{\mc{B}}$'s for $\mc{B} \geq 0$. If $\phi$
  indeed belongs to $\ebsS{\Sigma}$, then one of these
  procedures is guaranteed to terminate. The least $\mc{B}$ for which
  $\Xi_{\mc{B}}$ is valid gives the bound $\mc{B}$ for $\phi$ (since,
  if the bound for $\phi$ was lower, say $\mc{B}'$, then from the
  above proof, we know that $\Xi_{\mc{B}'}$ would have been valid thus
  violating the minimality of $\mc{B}$). It also gives an equivalent
  formula for $\phi$, namely $\psi_{\mc{B}}$, with the least number of
  $\exists^*$ quantifiers. This procedure thus requires us to
  construct \ti{exactly one} $\bsrS$ formula having
  $\mc{B} ~ \exists$ quantifiers for each $\mc{B}$ in order to find an
  equivalent $\bsrS$ formula for $\phi$. It just means
  that $\bsrS$ formulae other than the $\psi_{\mc{B}}$s
  need not be enumerated at all.



\item \ti{Uses in SAT and model checking:}An advantage of converting
  an $\ebsS{\Sigma}$ formula $\phi$ to its equivalent $\bsrS$ formula
  $\psi$ is that $\phi$ is satisfiable iff $\psi$ is
  satisfiable. There has been a lot of recent work ~\cite{bsr-sat} on
  decision procedures for the $\mathbf{EPR}$ class - which is the same
  as {\bsr}. While the fact that $\phi \in \ebsS{\Sigma}$ shows that the
  SAT-problem for $\ebsS{\Sigma}$ is decidable and the bound $\mc{B}$
  for $\phi$ gives a way of checking the satisfiability of $\phi$, we
  can leverage recent advances in decision procedures for {\bsr} to
  check for satisfiability of $\phi$.

  Likewise the model checking problem for $\phi$ (given a
  $\Sigma-$structure $M$, is it true that $M \models \phi$) would be
  the same as that for $\psi$.  Hence the power of model checkers
  optimized for {\bsr} ~could be leveraged.



\end{enumerate}




==> applicns.tex <==
\section{Spectral Properties of {\edpS{\emptyset}} and Applications}
\label{section:applicn}

Consider an {\edpS{\emptyset}} sentence
\[
\varphi = \forall \tbf{z}_0 \exists v_1 \forall \tbf{z}_1 \exists v_2 
\forall \tbf{z}_2 \ldots \exists v_r \forall \tbf{z}_r 
\xi(\tbf{z}, v_1 \ldots, v_r)
\]
where $\tbf{z} = (\tbf{z}_0, \ldots, \tbf{z}_r)$ and $\xi$ is
quantifier-free.  Let $\mc{B}$ be the bound for $\varphi$ as given by
Theorem~\ref{thm:edp-bound} (of section
\ref{subsection:proof_that_edp_is_a_frag_of_ebs}), and let $\mc{X} =
\{x_1, x_2, \ldots x_{\mc{B}}\}$ be a set of $\mc{B}$ fresh variables.
In addition, let $\psi$ be the {\bsrS} formula defined as follows.
\begin{tabular}{lll}
$\psi$ & = & $\exists x_1 \ldots \exists x_{\mc{B}} \forall \tbf{z}_0
\forall \tbf{z}_1 \ldots \forall \tbf{z}_r ~(\chi)~$ where\\
$\chi$ & = & $(\bigvee_{u_1 \in \mc{X}} \ldots \bigvee_{u_r \in \mc{X}} \xi
(\tbf{z}, v_1 \mapsto u_1, \ldots, v_r \mapsto u_r))$\\
\end{tabular}
where $\xi (\tbf{z}, v_1 \mapsto u_1, \ldots, v_r \mapsto u_r)$ is the
formula obtained by replacing every occurence of $v_i$ in $\xi$ by
$u_i$.

\begin{theorem}\label{thm:edp-equispectral-bsr}
The spectrum of $\varphi$ equals the spectrum of $\psi$.
\end{theorem}

\emph{Proof Sketch:} It is straightforward to see that every model of
$\psi$ is also a model of $\varphi$.  Therefore, the spectrum of
$\psi$ is contained in that of $\varphi$.  

For the other way round, consider a model $M$ of $\varphi$.  The
technique used in the proof of Theorem~\ref{thm:edp-bound} of section
\ref{subsection:proof_that_edp_is_a_frag_of_ebs} can now be used to
construct a model $M'$ of $\varphi$ such that $\mc{U}_M = \mc{U}_{M'}$
and $M \mid_\sigma = M' \mid_\sigma$.  Furthermore, the construction
guarantees that when $\varphi$ is evaluated on $M'$, all existentially
quantified variables can take values from a fixed subset $V \subset
\mc{U}_{M'}$ such that $|V| \leq \mc{B}$, and yet cause $\varphi$ to
evaluate to $\mathsf{True}$.  This special property of $M'$ ensures
that $M' \models \psi$ as well.  Since $\mc{U}_M = \mc{U}_{M'}$, this
proves that the spectrum of $\varphi$ is contained in the spectrum of
$\psi$.  Hence, $\varphi$ and $\psi$ have the same spectrum. Note that
$\psi$ is not semantically equivalent to $\varphi$.  It is certainly
equisatisfiable to $\varphi$, but is also ``equispectral'' to
$\varphi$.  \epf\\


An immediate application of Theorem~\ref{thm:edp-equispectral-bsr} in
SMT solving stems from recent results due to Fontaine~\cite{fontaine}.
In~\cite{fontaine}, a notion of \emph{gentle} theories is introduced
and it is argued that {\bsr}, L\"{o}wenheim and $FO^2$ ({\FO} with two
variables) theories are gentle.  Intuitively, a gentle theory is one
in which one can completely express the spectrum.  Fontaine further
shows that gentle theories can be combined with almost any other
decidable theories in an SMT solving setting with cooperating decision
procedures for multiple theories.  From
Theorem~\ref{thm:edp-equispectral-bsr}, we know that for every
$\varphi \in \edpS{\emptyset}$, we can effectively construct a {\bsr}
formula $\psi$ that has the same spectrum as $\varphi$.  Since {\bsr}
has been shown to be a gentle theory in~\cite{fontaine}, this implies
that {\edpS{\emptyset}} is gentle as well, and can be combined with
other decidable theories for SMT solving.  From
Theorem~\ref{thm:edp_lattice} (in section \ref{section:obs_on_edp})
and the fact that {\edpS{\Sigma}} contains {\bsrS}, we know that
{\edpS{\emptyset}} semantically generalizes {\bsrS}.  Hence,
{\edpS{\emptyset}} is a semantically richer theory than {\bsrS} that
is still gentle.  Interestingly, Fontaine gives separate proofs of
gentleness of the {\bsr} class and of the L\"{o}wenheim class with
equality~\cite{fontaine}.  Since L\"{o}weheim class with equality is
contained in {\ebsS{\Sigma}} with the bound $\mc{B} = q.2^k$ ($q =$
number of quantifiers, and $k =$ number of distinct monadic
predicates), Theorem~\ref{thm:lowest_EBS_equals_BSR} (of section
\ref{section:ebs_and_bsr}) and its proof
allow us to effectively construct a {\bsr} formula that is
semantically equivalent to a L\"{o}wenheim formula with equality.
Hence a gentleness proof of {\bsr} suffices to prove that the
L\"{o}wenheim class with equality is also gentle.
Section~\ref{subsection:lowenheim-with-equality} also describes how
{\edpS{\Sigma}} (and hence {\edpS{\emptyset}}) contains and indeed
generalizes the L\"{o}wenheim class with equality.  We, therefore,
believe that {\edpS{\emptyset}} and its variants truly expand the set
of gentle theories, and permit SMT solving with cooperating decision
procedures on richer problems.  Note that satisfiability checking for
formulas in {\edpS{\emptyset}} can be reduced to the satisfiability
checking problem of the equispectral {\bsrS} formula.  Model-finding
of {\edpS{\emptyset}} formulas can be done in the same way as is done
for {\bsrS} formulas~\cite{bsr-applns}.

Yet other interesting applications of the {\edpS{\emptyset}} class
arise in bounded model checking and inductive property checking.
Consider a (possibly infinite) state transition system whose
transition relation is given by a first order logic formula $T(s, s')$
on current and next state variables $s$ and $s'$ respectively.  Let
$I(s)$ and $P(s)$ be predicates on state variables denoting the
initial set of states and the set of states with property $P$.  In the
classical bounded model checking problem, we wish to find if there
exists a run of the system for $k$ steps, starting from an initial
state and ending in a state satisfying $P$.  This can be posed as
the satisfiability checking problem of the sentence:
\[
\varphi_{bmc} = \exists s_0\, \ldots \exists s_k\,\, I(s_0) \wedge T(s_0, s_1) \wedge \ldots T(s_{k-1}, s_k) \wedge P(s_k)
\]
Similarly, in inductive property checking, we wish to find if there
exists a run of the system for $k$ steps, starting from a state
satisfying $P$ such that $P$ is violated for the first time in the
$k^{th}$ step.  This is equivalent to checking the satisfiability of
the sentence:
\begin{eqnarray*}
\varphi_{ind} & = & \exists s_0\, \ldots \exists s_k\,\, P(s_0) \wedge T(s_0, s_1) \wedge P(s_1) \ldots \wedge \\
              &   &~~~~~~~~~~~~~~~~~~~~~ P(s_{k-1}) \wedge T(s_{k-1}, s_k) \wedge \neg P(s_k)
\end{eqnarray*}
It can be shown that if $I(s)$, $T(s, s')$, $P(s)$ and $\neg P(s)$ are
in {\edpS{\emptyset}}, then one can obtain the size of a bounded
model for both $\varphi_{bmc}$ and $\varphi_{ind}$ from the bounds
$\mc{B}$ for $I(s)$, $T(s, s')$, $P(s)$ and $\neg P(s)$.  The
``extensible'' bounded submodel property of {\edpS{\emptyset}}
formulae ensures that the bound of the model size for $\varphi_{bmc}$
and $\varphi_{ind}$ grows slowly (linearly) with $k$.  The reader is
referred to \cite{AS06} for further details.


==> conclusion.tex <==
\section{Conclusion}

In this paper, we presented a semantic and syntactic generalization of
the widely used {\bsr} class of first order logic sentences.  Our
study showed a lattice-structured generalization both in the semantic
and syntactic domains with strict inclusions between classes of
formulae.  The semantic generalization subsumes all {\FOS} formulae
with finite and co-finite spectra in the limit.  We also showed that
several well known decidable classes of {\FOS} sentences are subsumed
by our generalization.  This gives rise to alternative proofs of some
interesting results.  The syntactic generalization enjoys special
spectral properties, that can be effectively used in applications like
SMT solving, bounded model checking and inductive property checking.
There are several open questions that still remain.  Most important
among them is the question of whether a syntactic characterization of
{\ebsS{\emptyset}} is possible in the same sense that {\bsrS}
syntactically characterizes {\ebsS{\Sigma}.  Identifying other useful
fragments for which membership is decidable, and the bound $\mc{B}$ is
efficiently computable presents yet another major challenge for future
work.


==> ebs_empty.tex <==
\section{The $\ebsSempty$ class}\label{section:ebs_empty}

In this section, we study the \ebsSempty ~class. We firstly observe
that this class subsumes some well-known syntactic classes. 

\subsection{The $\ebsSempty$ class subsumes
  well-known syntactic classes} \label{subsection:obs_about_ebs_empty} 
We observe that for $\sigma = \emptyset$, the interpretations of none
of the predicates of $\Sigma$ are required to be preserved. We can
then easily see that the following lemma is true. Below cardinality of
a $\Sigma-$structure refers to the cardinality of its universe.
\begin{lemma} \label{lemma:ebs_empty_model_sizes}
A sentence $\varphi \in \ebsSempty$ iff either (i)
$\varphi$ is unsat or (ii) there exists a least finite
cardinal $\mc{B}$ such that $\varphi$ has a model of (a) every
cardinality $\geq \mc{B}$ if $\varphi$ has an infinite model and (b)
every cardinality ranging from $\mc{B}$ to the cardinality of
$\varphi$'s largest model if $\varphi$ has only finite models.
\end{lemma}

\ti{Proof}:

Suppose $\varphi \in \ebsSempty$. Let $\mc{B}$ be the bound for
$\phi$. Suppose it has an infinite model. We show that there is a
model of $\varphi$ of every cardinality $\geq \mc{B}$.

Take any finite cardinal $n \geq \mc{B}$. Since $\varphi$ has an
infinite model, by Compactness Theorem, there cannot be any bound on
the domain-size of the finite models of $\varphi$.  Then consider a
model $M$ of $\varphi$ of domain-size $\geq n$. Since $\varphi \in
\ebsSempty$, there exists $M_1 \subseteq M$
satisfying the $\ebsSempty$ conditions. Then take
any $M_2$ such that $M_1 \subseteq M_2 \subseteq M$ and
s.t. $|\mc{U}_{M_2}| = n$. Then there exists $M_2'$ such that $M_2'$
has the same domain as $M_2$ and $M_2' \models \varphi$. In other
words, there is a model of $\varphi$ of size $n$.

Take any infinite cardinal. Since $\varphi$ has an infinite model,
using the Upward and Downward L\"owenheim-Skolem theorems, we conclude
that there is a model of $\varphi$ of every infinite cardinality.

Summing up, $\varphi$ has models of every cardinality $\geq
\mc{B}$.\\

Suppose $\varphi$ has only finite models. Clearly then it cannot have
models of unbounded size because then by Compactness Theorem, it would
have an infinite model. Then there exists a finite cardinal $N$ such
that the domain-size of $\varphi'$s largest model is $N$.  Then by a
similar argument as above, we can show that $\varphi$ has models of
all domain-sizes ranging from $\mc{B}$ to $N$.


Thus the `only-if' part of the Lemma holds.\\

We now prove the `if' part. If $\varphi$ is unsatisfiable, $\varphi
\in \ebsSempty$ trivially.  Suppose $\varphi$ is
satisfiable and has an infinite model and there exists a smallest
finite cardinal $\mc{B}$ such that $\varphi$ has a model of every
cardinality $\geq \mc{B}$.  Take any model $M$ of $\varphi$ of
domain-size $\geq \mc{B}$. Consider any $M_1 \subseteq M$ such that
$|\mc{U}_{M_1}| = \mc{B}$. Consider any $M_2$ such that $M_1 \subseteq
M_2 \subseteq M$. Now from the premise, there exists a model $M_3$ of
$\varphi$ of cardinality $|\mc{U}_{M_2}|$. Then consider the
$\Sigma-$structure $M_2'$ which is isomorphic to $M_3$ and which has
universe $\mc{U}_{M_2}$. Since the set of models of $\varphi$ is
closed under isomorphism, $M_2' \models \varphi$ and is the desired
model. Thus $\varphi \in \ebsSempty$.

If $\varphi$ is satisfiable, has only finite models and has a model of
every cardinality ranging from $\mc{B}$ to the cardinality of
$\varphi$'s largest model, then by a similar argument as the one
above, we can show that $\varphi \in \ebsSempty$.

Thus the 'if' part holds as well proving the lemma. \epf\\



Using the above lemma, we can see that many well-known classes of
$\FOS$ sentences fall within $\ebsSempty$. It
can be shown that the following classes without functions but with
corresponding `function' predicates (i.e. we disallow functions but
allow in their place predicates which represent the functions by
including function axioms to be satisfied by the predicates) are also
inside $\ebsSempty$.
\begin{enumerate}
\item The L\"ob-Gurevich class - $\FOS$ without equality
  containing only unary predicates and only unary functions.
\item The Gurevich class - the set of all $\exists^*$ $\FOS$ sentences
possibly containing functions too.
\end{enumerate}

We prove the inclusion of the above classes in $\ebsSempty$ below.

\begin{lemma}\label{lemma:ebs_subsumes_lob_gurevich}
The L\"ob-Gurevich Class $\subseteq \ebsS{\emptyset}$
\end{lemma}

\ti{Proof:}

Consider the L\"ob-Gurevich Class.  This is the set of all $\FOS$
sentences without equality over a vocabulary which contains only unary
predicates and only unary function symbols.

As shown in ~\cite{BGG}(pp. 251), every sentence $\phi$ in the
L\"ob-Gurevich class is satisfiable over the same domains as a
L\"owenheim sentence $\psi$. Then $\phi$ and $\psi$ have the same
spectra. But we know that if signature of $\psi$ is $\Sigma$, then
$\psi \in \ebsSS \subseteq \ebsSempty$. Then using Lemma
\ref{lemma:ebs_empty_model_sizes} and the fact above that the spectrum
of $\phi$ is the same as that of $\psi$, we have that $\phi \in
\ebsS{\emptyset}$.

It is easy to see that a sentence in the L\"ob-Gurevich class, with
functions replaced by the corresponding function predicates satisfying
the function axioms will also be in $\phi \in \ebsS{\emptyset}$.\epf


\begin{lemma}\label{lemma:ebs_subsumes_gurevich}
The Gurevich Class $\subseteq \ebsS{\emptyset}$
\end{lemma}

\ti{Proof:}

Consider an $\FO$ sentence $\phi$ in the Gurevich class. Let
$\phi = \exists^* \tbf{z} \varphi (\tbf{z})$ where $\varphi$ could
contain function symbols and equality too in addition to
predicates. Suppose $M \models \phi$ such that $|\mc{U}_M| \geq
|\phi|$ where $|\phi|$ denotes the length of $\phi$. Then there exists
elements $\tbf{a}$ from $\mc{U}_M$ such that $M \models
\varphi(\tbf{a})$. Consider all the terms occuring in
$\varphi(\tbf{a})$. Let $\mc{T}$ be the set of all the values that
these terms evaluate to in $M$. Note that $|\mc{T}| < |\phi|$. Choose
an element $a^* \in \mc{U}_{M} \setminus \mc{T}$. Consider the model
$M'$ such that $\mc{U}_{M'} = \mc{U}_M$ and $M'|_{\mc{P}} =
M|_{\mc{P}}$ where $\mc{P}$ is the set of all predicate symbols of
$\Sigma$. Now for a $k-$ary function symbol $f \in \Sigma$, denote the
interpretations of $f$ in $M$ and $M'$ as $f_{M}$ and $f_{M'}$. Then
$f_{M'}$ is defined as follows: Let $f(t^1, \ldots, t^k)$ be a term in
$\varphi(\tbf{a})$. Let $t^1_M, \ldots t^k_M$ be the evaluations of
$t^1, \ldots, t^k$ in $M$ (then the former are values in
$\mc{T}$). Then $f_{M'}(t^1_M, \ldots, t^k_M) = f_M(t^1_M, \ldots,
t^k_M)$ (observe that this value must also be in $\mc{T}$). For all
other values $a_1, \ldots, a_k$ for which there do not exist terms
$t^1, \ldots, t^k$ such that (i) $t^i_M = a_i$ for $1 \leq i \leq k$
and (ii) $f(t^1, \ldots, t^k)$ is a term in $\varphi(\tbf{a})$, assign
$f(a_1, \ldots, a_k) = a^*$.

Then consider the substructure $M_1$ of $M'$ generated by $\mc{T} \cup
\{a^*\}$. One can see that by our construction above $\mc{U}_{M_1} =
\mc{T} \cup \{a^*\}$. Consider the substructure $M_2$ generated by any
$\mc{U}$ s.t. $\mc{U}_{M_1} \subseteq \mc{U} \subseteq \mc{U}_M$.
Again by our construction $\mc{U}_{M_2} = \mc{U}$. Then for all terms
$t$ appearing in $\varphi(\tbf{a})$, $t_{M_2} = t_{M'}$ (since $M_2
\subseteq M'$) and by construction $t_{M'} = t_M$. Then in $M_2$, all
the terms evaluate to exactly the same values as they evaluate to in
$M$. Now since $M_2|_{\mc{P}} = M'|_{\mc{P}} = M|_{\mc{P}}$ (the first
equality is because $M_2 \subseteq M'$ and the second is by
construction), $M_2 \models \varphi(\tbf{a})$ i.e. $M_2 \models \phi$.

This thus shows that given a model $M$ of $\phi$ of size $\geq \mc{B}
= |\phi|$, it is possible to construct a model $M'$ of $\phi$ by
preserving the interpretations of all the predicates of $\Sigma$ and
changing the interpretations of only the functions such that $M'$ has
the extensible bounded submodel property.

It is easy to see that $\Phi$ which is obtained by replacing the
functions in $\phi$ by their corresponding function predicates and
adding the function axioms will also satisfy the above property.

As a corollary of this we get that if $\Phi$ has a model with
domain-size $n \geq \mc{B}$, it has models of all domain-sizes ranging
from $\mc{B}$ to $n$. Then if $\Phi$ has models of unbounded
domain-size - which is iff it has an infinite model - then by the
previous statement and the Upward and Downward L\"owenheim-Skolem
theorems, it has models of all domain-sizes $\geq \mc{B}$. Thus $\Phi
\in \ebsSempty$ where $\Sigma$ is the vocabulary of $\Phi$.\epf\\


We have already seen earlier that $\FOS[1]$ and $\FOS[1]$ with
counting are inside $\ebsSS$ and hence inside $\ebsSempty$. We now
show below that $\FOS[2]$ ($\FOS$ with only two variables) is
contained in $\ebsSempty$.


\begin{lemma}\label{lemma:ebs_subsumes_FO[2]}
$\FOS[2] \subseteq \ebsSempty$
\end{lemma}

\ti{Proof:}

We refer to the proof of the finite model property of \FOS[2] as
shown in \cite{grakova97}. Firstly it is sufficent to consider only arity
$\leq 2$ predicates when dealing with \FOS[2]. As shown in \cite{grakova97},
an \FOS[2] sentence $\phi$ over $\Sigma$ is equisatisifiable over the
same domains with an \FOS[2] sentence $\psi$ over a vocabulary
$\Sigma_1$ which contains no arity $> 2$ predicates. The paper
further constructs a sentence $\theta$ over the same vocabulary
$\Sigma_1$, in Scott Normal Form. i.e. $\theta$ is of the form

\begin{tabular}{ll}
$\theta =$ & $ \forall x \forall y \alpha(x, y) \wedge~
\bigwedge_{i=1}^{i=m} \forall x \exists y (\beta_i(x, y) \wedge x \neq
y)$
\end{tabular}

where $\alpha$ and the $\beta_i$'s are quantifier-free. $\theta$ is
such that $\psi$ has a model whose domain-size is $n \geq 2$ iff
$\theta$ has a model with domain-size $n$. Then it is shown that if
$\theta$ is satisfiable, it has a model with domain-size atmost
$3m.2^n$ where $n = |\Sigma_1|$.

We now show that if $\theta$ is satisfiable, either it has only
finitely many models or it has models with all domain-sizes $\geq
3m.2^n$. Then $\psi$ and hence $\phi$ would have either finitely many
models or models with all domain-sizes $\geq 3m.2^n$.  The argument is
a simple extension of the procedure (given in \cite{grakova97}) used in
constructing the small model for $\theta$.


Firstly if all models of $\theta$ have domain-size $\leq 2^n$ then all
models of $\psi$ and hence $\phi$ would also have domain-size $\leq
2^n$. If not then consider a model of $\theta$ of domain size $>
2^n$. Then there exists an element in the model which is not a `king'
(See ~\cite{grakova97} for the definition of 'king'). Now from this model,
construct the small model $M$ for $\theta$ as per the procedure. Then
in $M$ consider an element $d_{ij}$ (using the same notation as in the
paper). We introduce a new element $d'$ in $M$ which will `mimic'
$d_{ij}$. In particular, $d'$ has the same 1-type as $d_{ij}$. Next,
for every element $e$ in $M$ different from $d_{ij}$ and $d'$, we make
the 2-type of $(d', e)$ the same as the 2-type of $(d_{ij}, e)$.  Note
that this 2-type assignment cannot cause a conflict for the 1-type of
$e$ or for the 1-type of $d'$. Further this assignment of the 2-type
between $d'$ and $e$ cannot conflict with the 2-types of the already
existing (i.e. prior to the introduction of $d'$) pairs of elements
since this 2-type is being assigned for a completely new pair of
elements.  Finally assign the 2-type of $(d', d_{ij})$ to be the
2-type of any two elements of $M$ whose 1-types are the same as that
of $d'$ and $d_{ij}$, for example say, $e_{ij}$ and $d_{ij}$. Thus
there would be no conflicts at all in this new structure, call it
$M^{+}$.

Now we show that $M^+ \models \theta$. While the existing elements
already have `skolem witnesses', it remains to choose skolem witnesses
for $d'$. To provide skolem witnesses for $d'$, we will again just
mimic what was done for $d_{ij}$ i.e. for each $k \in \{1, \ldots,
m\}$, we will choose the same skolem witness for $d'$ for $k$ as the
the skolem witness $g_k(d_{ij})$ for $d_{ij}$ for $k$.  Now by
construction, the 2 types of $(d_{ij}, g_k(d_{ij}))$ and $(d',
g_k(d_{ij}))$ are the same.  Since the 2-type of $(d_{ij},
g_k(d_{ij}))$ ensures that $\beta_k(d_{ij}, g_k(d_{ij}))$ was
$\mathsf{True}$, $\beta_k(d', g_k(d_{ij}))$ will also be
$\mathsf{True}$. Then the second conjunct above of $\theta$ would be
true in $M^+$. Since the 2-type between $d'$ and any element $e$ of
$M$ is one that was already existing in $M$ and since the first
conjunct of $\theta$ was true in $M$, the first conjunct would be true
in $M^+$ as well. Then $M^+ \models \theta$. Note that $|\mc{U}_{M^+}|
= |\mc{U}_M| + 1$.

We can now use the same procedure on $M^+$ to get another model of
$\theta$ which contains one more element than the number of elements
in $M^+$ and so on. Thus $\theta$ has models with all domain-sizes
$\geq 3m.2^n$ since the initial model $M$ had domain-size $\leq
3m.2^n$. Then back-tracking, $\psi$ and hence $\phi$ has models with
all domain-sizes $\geq 3m.2^n$.

Thus $\phi$ is either unsatisfiable, or has finitely many models (all
having domain-size $\leq 2^n$) or has models with all domain-sizes
$\geq 3m.2^n$. Then by Lemma \ref{lemma:ebs_empty_model_sizes}, $\phi
\in \ebsSempty$ with $\mc{B} \leq 3m.2^n$.\epf\\


It can also be shown easily that the class of all $\FOS$ sentences
without equality which have the finite model property is
contained inside $\ebsSempty$.


\begin{lemma}\label{lemma:ebs_subsumes_FO_without_equality_with_FMP}
$\FOS$ without equality and with finite model property $\subseteq
\ebsS{\emptyset}$
\end{lemma}

\ti{Proof:}

It is well known that if an $\FOS$ without equality sentence $\phi$
has a model of size $n$, then it also has a model of size $n+1$. Then
if $\phi$ has finite model property, then either $\phi$ is
unsatisfiable or there exists a least $\mc{B}$ s.t. $\phi$ has models
of all cardinalities $\geq \mc{B}$. Then from Lemma
\ref{lemma:ebs_empty_model_sizes}, $\phi \in \ebsS{\emptyset}$.\epf\\



Any $\ebsSempty$ sentence (and hence one without equality) has the
finite model property. This shows that \\

\begin{tabular}{lll}
\ebsSempty & = & {\FOS} without equality and \\
& & with finite model property\\
\end{tabular}\\

An example of an $\FOS$ without equality subclass with finite model
property is the G\"odel-Kalm\'ar-Sch\"utte class over $\Sigma$ which
is the set of all $\exists^* \forall \forall \exists^*$ $\FOS$
sentences without equality. This class has the small model property
(see ~\cite{BGG}). Then this class is contained inside $\ebsSempty$.


\subsection{An interesting property of $\ebsS{\emptyset}$ without equality}
\label{subsection:interesting_property_of_ebs_empty}

Consider a sentence $\phi \in \ebsSempty$ without equality. Given a
model $M$ of $\phi$ of domain-size $\geq \mc{B}$ where $\mc{B}$ is the
bound for $\phi$, it is not necessary that $M$ have a bounded core all
of whose extensions within $M$ also satisfy $\phi$. But interestingly,
we show in this section that one can always get another model $M'$
with the same universe as that of $M$ such that $M'$ has a bounded
core (of size $\leq \mc{B}$) all of whose extensions within $M'$ are
also models of $\phi$.


Consider a satisfiable sentence $\phi \in \ebsS{\emptyset}$ without
equality. Then there exists a $\mc{B}$ for $\phi$ such that for all
domain sizes $n \geq \mc{B}$ we can construct a model $M$ of
domain-size $n$. Then there exists a model $\hat{M}$ of $\phi$ of
domain-size $\mc{B}$. Then it is possible to construct an isomorphic
model $M^*$ whose universe is $\mc{U}_{M^*} = \{a_1, \ldots,
a_{\mc{B}}\} \subseteq \mc{U}_M$. Then $M^* \models \phi$. We will use
this model to construct the desired $M'$. Let $f:\mc{U}_M \rightarrow
\mc{U}_{M^*}$ be any function from $\mc{U}_M$ to $\mc{U}_{M^*}$ such
that $f(a_i) = a_i$ for all $i \in \{1, \ldots, \mc{B}\}$. For each
$k-$ary predicate $P \in \Sigma$, denote the interpretation of $P$ in
$M'$ and $M^*$ as $P^{M'}$ and $P^{M^*}$ respectively. Then define $P$
in $M'$ such that $M' \models P(b_1, \ldots, b_k) ~\textrm{iff}~ M^*
\models P(f(b_1), \ldots, f(b_k))$ for $b_1, \ldots, b_k \in
\mc{U}_M$. Let w.l.o.g., $\phi$ be given by
\[
\phi = \forall \tbf{z}_0 \exists v_1 \forall \tbf{z}_1 \exists v_2 
\forall \tbf{z}_2 \ldots \exists v_r \forall \tbf{z}_r 
\xi(\tbf{z}, v_1 \ldots, v_r)
\]
where $\tbf{z} = (\tbf{z}_0, \ldots, \tbf{z}_r)$ and $\xi$ is
quantifier-free and in CNF. We will show that $M' \models \phi$.

Consider an instantiation $\mc{Z}$ of $\tbf{z}$ from $\mc{U}_{M'} =
\mc{U}_M$. We need to choose values $d_1, \ldots, d_r$ for the
variables $v_1, \ldots v_r$ such that $M' \models \xi(\mc{Z}, d_1,
\ldots, d_r)$. Let $\mc{Z}^*$ be the vector of values obtained by
subjecting $\mc{Z}$ to $f$ component-wise. Then $\mc{Z}^*$ is a vector
of values from $\mc{U}_{M^*}$. Now since $M^* \models \phi$, there
exist values $d_1^*, \ldots, d_r^*$ from $\mc{U}_{M^*}$ such that $M^*
\models \xi(\mc{Z}^*, d_1^*, \ldots, d_r^*)$. Then for each $i \in
\{1, \ldots, r\}$ choose $d_i = d_i^*$. Now consider an instance of
$P$ in $\xi(\mc{Z}, d_1, \ldots, d_r)$. Say it is $P(e_1, \ldots,
e_k)$. Then by construction above $M' \models P(e_1, \ldots, e_k)
~\textrm{iff}~ M^* \models P(f(e_1), \ldots, f(e_k))$. But since
$\mc{Z}^*$ is the image of $\mc{Z}$ under $f$ and $f(d_i) = f(d_i^*) =
d_i^*$, we find that $P(f(e_1), \ldots, f(e_k))$ is the corresponding
instance of $P(e_1, \ldots, e_k)$ in $\xi(\mc{Z}^*, d_1^*, \ldots,
d_r^*)$. Then since the latter is $\mathsf{True}$ in $M^*$,
$\xi(\mc{Z}, d_1, \ldots, d_r)$ is $\mathsf{True}$ in $M'$. Since
$\mc{Z}$ was arbitrary, $M' \models \phi$.

Now let $M_1$ be the substructure of $M'$ generated by $\{a_1, \ldots,
a_{\mc{B}}\}$. Let $M_1 \subseteq M_2 \subseteq M'$. Then since $M_2
\subseteq M'$, for each $k-$ary $P \in \Sigma$, $M_2 \models P(b_1,
\ldots, b_k) \leftrightarrow M' \models P(b_1, \ldots, b_k)
\leftrightarrow M^* \models P(f(b_1), \ldots, f(b_k))$. Then by a
similar argument as the one shown above, we can infer that $M_2
\models \phi$. Thus $M'$ has the extensible bounded core property
where the core has domain-size $\leq \mc{B}$.\\

Interestingly, in the above construction, we note that in making
$\phi$ $\mathsf{True}$ in $M_2$, the `inner' existential variables
always take values from a fixed set of size $\mc{B}$, namely $\{a_1,
\ldots, a_{\mc{B}}\}$. Then we construct the formula $\psi$ as
given in the proof of Theorem \ref{thm:lowest_EBS_equals_BSR} (in
section \ref{section:ebs_and_bsr}) i.e.

\begin{tabular}{lll}
$\psi$ & = & $\exists x_1 \ldots \exists x_{\mc{B}} \forall \tbf{z}_0
\forall \tbf{z}_1 \ldots \forall \tbf{z}_r ~(\chi)~$ where\\
$\chi$ & = & $(\bigvee_{u_1 \in \mc{V}} \ldots \bigvee_{u_r \in \mc{V}} \xi
(\tbf{z}, v_1 \mapsto u_1, \ldots, v_r \mapsto u_r))$\\
\end{tabular}

Then we can see that on account of the extensible bounded core
property of $M'$, $M' \models \psi$. As shown above, for \ti{any}
model $M$ of domain-size $\geq \mc{B}$, we can construct a model $M'$
having the same domain as $M$ and which has the extensible bounded
core property. Then the spectrum of $\phi$ is a subset of the spectrum
of $\psi$. Clearly it is the case that if $M \models \psi$, then $M
\models \phi$. Then the spectrum of $\psi$ is a subset of the spectrum
of $\phi$. Then we conclude that $\phi$ and $\psi$ have the same
spectrum. Thus we can answer any questions regarding the spectrum of
$\phi$ by just asking the same questions of the spectrum of $\psi$
which is a $\bsrS$ sentence.



While we do not know whether this property extends to the whole of
$\ebsSempty$ with equality, in some cases it
does. Consider a sentence $\phi$ in the Gurevich class seen above. As
shown in the proof of Lemma \ref{lemma:ebs_subsumes_gurevich}, for
every model $M$ of $\phi$, as above, one can construct $M'$ by
changing only the interpretations of the `function' predicates (and by
keeping the interpretations of the other predicates as in $M$) such
that $M'$ has the above mentioned extensible bounded core property.

\subsection{The SAT problem for the $\ebsSempty$ class}
\label{subsection:sat_problem_for_ebs_empty}

\begin{lemma} \label{lemma:ebs_sat_is_decidable}
If $\varphi \in \ebsSempty$, the following problems
are decidable:\\ 
(i) Is $\varphi$ satisfiable?\\ 
(ii) Does $\varphi$ have a finite model?
\end{lemma}

\emph{Proof:} By Lemma~\ref{lemma:ebs_empty_model_sizes}, if $\varphi
\in \mc{EBS}$, it is either unsatisfiable or has a finite model of
size atmost $\mc{B}$, where $\mc{B}$ is the finite cardinal in
Lemma~\ref{lemma:ebs_empty_model_sizes}.  By Herbrand's theorem, if
$\varphi$ is unsatisfiable, there must exist a finite set of ground
clauses of $\varphi$ that is propositionally unsatisfiable.  We can
therefore construct a decision procedure by interleaving steps of the
following:
\begin{itemize}
\item A procedure that recursively enumerates the ground clauses in
the Herbrand Universe of $\varphi$ and checks the propositional
unsatisfiability of finite subsets of ground clauses, and
\item A procedure that recursively enumerates finite models of
$\varphi$ and checks whether $\varphi$ is true in the model.
\end{itemize}
Since $\varphi$ is either unsatisfiable or has a finite model of size
at most $\mc{B}$, one of these is guaranteed to terminate.  If we
terminate by detecting unsatisifability of $\varphi$, then $\varphi$
has no model.  Otherwise, we terminate with a finite model of
$\varphi$.  This gives us a decision procedure that serves to check
satisfiability of $\varphi$ and also detects if $\varphi$ has a finite
model.\epf \\


Now $\bsrS \subseteq \ebsSS \subseteq \ebsSs$ for $\sigma \subseteq
\Sigma$. Since the SAT problem for $\bsrS$ is
{\sc{NExpTime}}-complete, the SAT problem for $\ebsSs$ for any $\sigma
\subseteq \Sigma$ (and in particular $\sigma = \emptyset$), is atleast
{\sc{NExpTime}}-hard.

For some special subclasses of $\ebsSempty$, we identify below the
complexity of the SAT problem for these subclasses. 
 

\begin{lemma}\label{lemma:SAT_complexity_of_subclass_of_ebs}
Assume a sub-class $\mc{S}$ of $\ebsSempty$ for which $\mc{B}$ for
every sentence $\phi$ of the sub-class is atmost $f(\phi)$ where $f:
\mc{S} \rightarrow \mathbb{N}$ is an efficiently (polynomial time)
computable function. Then $\textrm{SAT-}\mc{S} \in
\textrm{\sc{NTime}}(f(\phi)^{O(|\phi|)})$ where $\textrm{SAT-}\mc{S}$
denotes the SAT problem for $\mc{S}$ and $|\phi|$ denotes the length
of $\phi$.
\end{lemma}

\ti{Proof}:

Given a formula $\phi \in \mc{S} \subseteq \ebsS{\emptyset}$, we
construct a Turing machine which does the following:
\begin{enumerate}
\item It first brings $\phi$ to its PCNF $\varphi$. The time taken to
  do so is $O(|\phi|)$. The length of $\varphi$, i.e. $|\varphi| =
  O(|\phi|)$.
\item It computes $\mc{B} = f(\phi)$. The time taken for this is
  $O(q(|\phi|))$ where $q$ is some polynomial.
\item It then guesses a number $n$ between $0$ and $\mc{B}$. It then
  constructs the set $\{1, \ldots, n\}$ which would serve as the
  universe $\mc{U}_M$ of a $\Sigma-$structure $M$. The time required
  to construct the universe is $O(n) = O(\mc{B})$.
\item It then guesses the $\Sigma-$structure $M$. Let $r$ be the
  number of predicates in $\phi$ ($r = O(|\phi|)$). Let $s$ be the
  maximum arity of these predicates ($s = O(|\phi|)$. To interpret any
  predicate $P$ requires specifying the truth value of $P$ for each
  $s-$tuple of arguments from $\mc{U}_M$. Then the time required to
  guess an interpretation of $P$ is $O(n^s)$. Doing so for all
  predicates requires time $O(r \cdot n^s) = O(|\phi| \cdot
  n^{|\phi|})$. Thus the time to guess the $\Sigma-$structure $M$ is
  $O(|\phi| \cdot n^{|\phi|})$. This also is the size of $M$ which we
  denote by $\parallel M \parallel$ i.e. $\parallel M \parallel =
  O(|\phi| \cdot n^{|\phi|})$.
\item It then checks whether $M \models \varphi$. It does so by
  enlisting out all the matrices obtained by instantiating the
  variables in the matrix of $\varphi$ with values from $\mc{U}_M$ and
  then checking whether these instantiated matrices evaluate to
  $\mathsf{True}$ in $M$. Given an instantiated matrix, the time
  required to check whether the matrix is $\mathsf{True}$ in $M$ is
  $O(\parallel M \parallel \cdot ~|\varphi|)$ = $O(\parallel M
  \parallel \cdot ~|\phi|)$. If the length of the quantifier prefix of
  $\varphi$ is $p (= O(|\varphi|) = O(|\phi|))$, then the number of
  instantiated matrices is $O(n^p)$. Then the total time to check
  whether $M \models \varphi$ is $O(n^p) \cdot O(\parallel M \parallel
  \cdot ~|\phi|) = O(n^{|\phi|} \cdot |\phi| \cdot n^{|\phi|} \cdot
  |\phi|) = O( n^{2 \cdot |\phi|} \cdot |\phi|^2)$. 
\end{enumerate}
If $M \models \varphi$, then the TM returns $\mathsf{Yes}$
(i.e. $\varphi$ and hence $\phi$ is satisfiable and also would have
constructed the model $M$ satisfying it).  If all computations of $M$
fail, then it indeed must be that $\varphi$ and hence $\phi$ is
unsatisfiable due to the bounded model property of $\phi$. Thus $M$
decides the satisfiability of $\phi$. \\

The time taken for any computation =

Time to compute $\varphi$ (A) + Time to compute $f$ (B) + Time taken to guess
  $n$ (C) + Time taken to guess $M$ with universe of size $n$ (D) + Time
  taken to check if $M \models \varphi$ (E) \\


Now (C) + (D) + (E) 

\begin{tabular}{ll}
=~~ & $O(n)$ + $O(|\phi| \cdot n^{|\phi|})$ +
  $O( n^{2 \cdot |\phi|} \cdot |\phi|^2)$ \\
=~~ & $O( n^{2 \cdot |\phi|} \cdot |\phi|^2)$\\
=~~ & $O( n^{O(|\phi|)})$\\
\end{tabular}

Then (A) + (B) + (C) + (D) + (E) 

\begin{tabular}{ll}
=~~ & $O(|\phi|)$ + $O(q(|\phi|))$ + $O( n^{O(|\phi|)})$\\
=~~ & $O( n^{O(|\phi|)})$\\
=~~ & $O( f(\phi)^{O(|\phi|)})$\\
\end{tabular}

Thus $\textrm{SAT-}\mc{S} \in
\textrm{\sc{NTime}}(f(\phi)^{O(|\phi|)})$. \epf\\

We get the following immediately as a consequence of the above Lemma.

\begin{Corollary}
\label{corollary:nexptime_SAT_complexity_of_subclass_of_ebs}
If for the sub-class $\mc{S}$ satisfying the conditions of Lemma
\ref{lemma:SAT_complexity_of_subclass_of_ebs}, $f(\phi) \leq
2^{p(|\phi|)}$ for some polynomial $p$, then $\textrm{SAT-}\mc{S} \in
\textrm{\sc{NExpTime}}$. If $S$ contains $\bsrS$, then SAT-$\mc{S}$ is
{\sc{NExpTime}}-complete.
\end{Corollary}


We shall look at one such class as stated in the above lemma later in
section \ref{section:edp}).



==> ebs_intro.tex <==
\section{The $\ebsSs$
  class}\label{section:ebs_sigma_introduction}

\begin{defn}[The $\ebsSs$ class]\label{def:ebs_general}
Let $\varphi$ be an {\FOS} sentence.  Then $\varphi$ is said to
have the \tbf{Extensible Bounded Sub-Model} property preserving
$\sigma \subseteq \Sigma$ if the following holds:

There exists a least finite cardinal $\mc{B}$ (called the \ti{bound
for $\varphi$} - dependent on $\varphi$ and $\sigma$ in general) such
that for every $\Sigma-$structure $M$, if $M \models \varphi$, then
there exists a sub-structure $M_1$ of $M$ such that
\begin{enumerate}
\item $|\mc{U}_{M_1}| \leq \mc{B}$ \label{ebs_general:cond2}
\item \label{ebs_general:cond3} For every extension $M_2$ of $M_1$
within $M$, there exists a $\Sigma-$structure $M_2'$ such that
$\mc{U}_{M_2} = \mc{U}_{M_2'}$, $M_2' \models \varphi$ and
$M_2'|_{\sigma} = M_2|_{\sigma}$.
\end{enumerate}

The set of all {\FOS} sentences having the extensible bounded
sub-model property preserving $\sigma$ is called the
$\ebsSs$ class.
\end{defn}

We will encounter examples of formulae in the above family of classes
in the forthcoming sections. We organize our study of 
$\ebsS{\sigma}$ into three parts in the sequel: (a) The case when $\sigma =
\Sigma$ (b) The case when $\sigma$ is not necessarily restricted to
$\Sigma$ (c) The case when $\sigma = \emptyset$. 


==> ebs_undec.tex <==
\section{Undecidability of the $\ebsSs$ classes}\label{section:ebs_undec}

While the satisfiability problem for $\ebsSs$ is decidable, the
membership problem for $\ebsSs$ is not always decidable. Below we look
at the cases where $\ebsSs$ is decidable and where it is
undecidable. In the latter case, we show a reduction from the halting
problem.

As shown in ~\cite{survey-on-dec-and-undec-of-halting-problem}, while
the set of all those TMs which halt on the empty tape is undecidable,
researchers set out to find out subsets of this set, which are
undecidable. For any pair $(s, l)$ of natural numbers, define the set
$\mc{A}_{(s, l)}$ to be the set of all the TMs having $s+1$ states
(including the halting state) and $l$ symbols (including the blank
symbol).  Then it can be shown
(~\cite{survey-on-dec-and-undec-of-halting-problem}) that if
$\mc{A}_{(s, l)}$ is undecidable, then $\mc{A}_{(x, y)}$ is
undecidable for $s \leq x$ and $l \leq y$. A set $R$ of seven such
pairs $(s, l)$ have been identified
(~\cite{survey-on-dec-and-undec-of-halting-problem}) such that
$\mc{A}_{(s, l)}$ is undecidable and further these are such that there
remain only a fixed finite number of pairs $(x, y)$ for which the
decidability status of $\mc{A}_{(x, y)}$ is unknown. We use this set
$R$ in the theorem below.


\begin{theorem}\label{thm:ebs_undec}
For any $\sigma \subseteq \Sigma$,
\begin{enumerate}
\item If $\Sigma$ contains only unary predicates,
$\ebsSs$ is
decidable.\label{theorem:ebs_undec:all_unary}
\item If $\Sigma$ contains at least $s+1$ unary predicates and atleast
$l+1$ predicates of arity $\geq 2$, where $(s, l) \in R$, then
$\ebsSs$ is undecidable.\label{theorem:ebs_undec:some_non-unary}
\end{enumerate}
\end{theorem}


\emph{Proof:}

Statement (1) above is easy to see. If $\Sigma$ contains only unary
predicates, then as seen earlier, $\ebsSs = \ebsSS =
\FOS$. Then checking membership is trivial.

We now consider statement (2) above. Consider the pair $(s, l)$. Then
as mentioned above, $\mc{A}_{(s, l)}$ is undecidable. We show a
reduction from $\mc{A}_{(s, l)}$ to the set $\overline{\ebsSs}$ which
is the complement of the set $\ebsSs$. Clearly $\overline{\ebsSs}$ is
decidable iff $\ebsSs$ is decidable.


Consider $\mc{M}_1 \in \mc{A}_{(s, l)}$. Let $\mc{M}_1 = (Q, \Sigma,
\Delta, \delta_1, q_0, \left\{ h \right\})$ be a deterministic Turing
Machine (DTM) with a two-way infinite tape, where $Q$ is the set of
states such that $|Q| = s+1$, $\Sigma$ represents the input alphabet,
$\Delta$ represents the tape alphabet such that $|\Delta| = l$,
$\delta_1: Q \times \Delta \rightarrow Q \times \Delta \times \{L,R\}$
represents the deterministic transition function, $q_0$ represents the
starting state and $h$ represents the unique halting state.

We first modify $\mc{M}_1$ to a new DTM $\mc{M} =
(Q\cup\left\{t\right\}, \Sigma, \Delta, \delta, q_0, \emptyset)$,
where $t \not\in Q$ and

$\delta(q,i) = \delta_1(q,i), \forall q \in Q \setminus \{h\}, \forall
i \in\Delta;~~$

$\delta(h,i) = (t,i,R),~~\delta(t,i) = (h,i,L) ~~~\forall i \in \Delta$\\

Thus $\mc{M}$ mimics the behaviour of $\mc{M}_1$ exactly except when
$\mc{M}_1$ reaches the halting state $h$.  On reaching this state,
$\mc{M}$ loops between states $h$ and $t$ forever.  Note that $\mc{M}$
does not have a halting state.


Next, we construct a sentence $\Phi_\mc{M} \in \FOS$ such that
models of $\Phi_\mc{M}$ represent computations of $\mc{M}$ on the
empty input tape that end in state $t$. For this, we proceed exactly
as in the proof of Trakhtenbrot's theorem as presented in~\cite[pp
165-168]{LL98} (details are therefore omitted here). We make the
following slight changes though.
\begin{enumerate}
\item The proof in ~\cite{LL98} uses only binary predicates whereas
the arity $\geq 2$ predicates of $\Sigma$ need not necessarily be
binary. But it is easy to see that binary predicates can always be
simulated using higher arity predicates (as was shown earlier in
section \ref{subsection:lattice_structures}).
\item The proof in ~\cite{LL98} introduces a binary predicate $H_q(p,
n)$ for each state $q$ where $H_q(p, n)$ denotes that at time $n$,
$\mc{M}$ is in state $q$ and its head is at position $p$ on the
tape. We instead separate the state and the head-position information
by using a unary predicate $U_q(n)$ for each state $q \in Q$ and a
arity $\geq 2$ predicate $H$. $H(p, n, \ldots, n)$ is $\mathsf{True}$
iff the head is at position $p$ at time $n$. $U_q(n)$ denotes that
$\mc{M}$ is in state $q$ at time $n$. If for a given $n$, all
$U_q(n)$'s are $\mathsf{False}$, it would be taken to mean that at
time $n$, $\mc{M}$ is state $t$. The constraints can easily be recast
in terms of these predicates. The total number of unary predicates
needed above is $s+1$ - which is possible to use from $\Sigma$ since
$\Sigma$ contains atleast $s+1$ unary predicates.
\item The proof in ~\cite{LL98} uses the constant
$\underline{\textrm{min}}$. We get rid of this constant and replace
 all its occurences with a variable say $x$ which will be
 existentially quantified. Since $\mc{M}$ uses a two-way infinite
 tape, we remove the constraint that $x$ is the minimum element. $x$
 would just be some element which would represent the start time.
\item The proof in ~\cite{LL98} considers the tape alphabet to be
 $\{0.1\}$. But the same constraints as for this tape alphabet, can be
 written for any general tape alphabet, in particular $\Delta$. Then
 one binary predicate $P_a(p, n)$ would be used for each $a \in
 \Delta$ with the constraint that for any $(p, n)$ exactly one these
 predicates is $\mathsf{True}$. That requires $l$ binary predicates
 for all symbols together. But we use only $l-1$ arity $\geq 2$
 predicates - one predicate $P_a$ for each symbol in $\Sigma$ and
 assert that \ti{atmost} one such predicate is $\mathsf{True}$ for
 each $(p, n)$. The case when all the $P_a$'s are $\mathsf{False}$
 will be taken to mean that the blank symbol is present at position
 $p$ at time $n$. The total number of arity $\geq 2$ predicates needed
 would be $l-1$ (for the $P_a$ predicates) + $1$ (for $H$) + $1$ (for
 the linear order) = $l+1$. These can be used from $\Sigma$ since
 $\Sigma$ contains alteast $l+1$ arity $\geq 2$ predicates.
\item The proof in ~\cite{LL98} assumes a complete DTM. Here we do not
 require it to be so. Hence we need to capture the condition that
 $\mc{M}$ might halt on a state $q$ - which is not the halting state -
 just because there is no transition out from the state on the symbol
 $a$ currently under the head (Clearly the input is not accepted by
 this halting). Then we add the following constraint $\phi$ in
 $\Phi_1$ for each such $q$ and $a$:

$\textrm{last}(y) = \forall x ((x \neq y) \rightarrow (x < y))$ 

$\phi(y) =\forall n \forall p ( (U_q(n) \wedge H(p, n, \ldots, n)
\wedge P_a(p, n, \ldots, n)) \rightarrow \bigvee_{q \in Q}
U_q(\textrm{last}(y)))$

 where $P_a(p, n, \ldots, n)$ is $\mathsf{True}$ iff at time $n$, the
 symbol at position $p$ on the tape is $a$. $\phi$ then asserts that
 if $q$ and $a$ are as mentioned above, the last state of the
 computation is not $t$.
\item The last condition is changed to assert that the last state of
the computation is $t$

$\Phi_2 = \exists x (\textrm{last}(x) \wedge \bigwedge_{q \in Q} \neg
U_q(x))$.


\item For all those $P \in \Sigma$ which were not used in the
constraints above, we just add the constraint $\psi_P = \forall
\tbf{z}_P P(\tbf{z}_P)$ where $\tbf{z}_P$ is a vector of length equal
to the arity of $P$. These additional constraints are just to make
$\Phi_{\mc{M}}$ have signature equal to $\Sigma$.
\end{enumerate}

The above constructed $\Phi_{\mc{M}}$ can be seen to be in
$\FOS$. We now observe that.
\begin{enumerate}[A)]
\item A $\Sigma-$structure $M$ with $|\mc{U}_M|=\alpha$ for some
cardinal $\alpha$ is a model of $\Phi_\mc{M}$ iff $M$ represents a
computation of length $\alpha$ of the DTM $\mc{M}$ (on the empty input
tape) which ends in state $t$.  \label{L10}
\end{enumerate}

We now show that $\mc{M}_1$ halts on the empty input tape iff
$\Phi_\mc{M} \in \overline{\ebsSs}$.

\noindent \emph{\bfseries If part:} Suppose $\mc{M}_1$ does not halt
at the halting state $h$. Then $\mc{M}$ either halts at a non-halting
state or it has an infinite computation that does not through $t$. In
either case, no computation of it ends in $t$. Since by (\ref{L10})
above, there is a 1-1 correspondance between computations of $\mc{M}$
that end in state $t$ and the models of $\phi_{\mc{M}}$, we find that
$\phi_{\mc{M}}$ is unsatisfiable. Then $\phi_{\mc{M}} \in \ebsSs$
trivially. So $\phi_{\mc{M}} \notin \overline{\ebsSs}$.

\noindent \emph{\bfseries Only if part:} Suppose that $\mc{M}_1$ halts
at the halting state $h$. Let $\mc{N}$ be the length of the `halting'
computation of $\mc{M}_1$. Then $\mc{M}$ reaches $h$ for the first
time after $\mc{N}$ steps. We have the following two observations:
\begin{enumerate}
\item\label{L20} 
Consider the computation of $\mc{M}$ of length $\mc{N}+2k ~(k \ge 0)$
(since $\mc{M}$ is a DTM, there is only one computation of length
$\mc{N} + 2k$ for each $k$).  By the construction of $\mc{M}$, every
such computation ends in state $h$ (and hence not at $t$). Then from
observation (\ref{L10}) above, $\Phi_{\mc{M}}$ has no model of size
$\mc{N} + 2k$ for all $k\geq 0$.
\item \label{L21} 
Consider the computation of $\mc{M}$ of length $\mc{N}+2k+1 ~(k \ge
0)$.  By construction, the computation ends in state $t$. Then by
(\ref{L10}) above, there exists a model of $\Phi_M$ of size
$\mc{N}+2k+1$, for every $k \ge 0$.
\end{enumerate}

Suppose that $\Phi_\mc{M} \in \ebsSempty$.  From observation
(\ref{L21}), we know that $\Phi_{\mc{M}}$ has infinitely many models.
Then by Lemma~\ref{lemma:ebs_empty_model_sizes} (in section
\ref{subsection:obs_about_ebs_empty}), there exists a finite cardinal
$\mc{B}$ such that $\Phi_{\mc{M}}$ has a model of every size larger
than $\mc{B}$.  However, from observation~(\ref{L20}), we know that by
taking any $k$ such that $\mc{N} + 2k > \mc{B}$, $\Phi_M$ has no model
of size $\mc{N} + 2k$.  Therefore, $\Phi_\mc{M} \notin
\ebsSempty$. Then since $\ebsSs \subseteq \ebsSempty$ we conclude that
$\Phi_\mc{M} \in \overline{\ebsSs}$.


Thus $\mc{M}_1$ halts iff $\Phi_M \in \overline{\ebsSs}$. Thus
$\overline{\ebsSs}$ is undecidable. Hence $\ebsSs$ is
undecidable.\epf\\






The above proof ofcourse leaves out the $\Sigma$s which contain $s+1$
unary predicates and $l+1$ predicates of arity $\geq 2$ where the
decidability status of $\mc{A}_{(s, l)}$ is unknown. We do not have an
answer yet for the decidability of $\ebsSs$ for these $\Sigma$s but we
conjecture that these must be undecidable as well.

While for the $\Sigma$s considered in Theorem
\ref{thm:ebs_undec}(\ref{theorem:ebs_undec:some_non-unary}), the
latter says that $\ebsSs$ is undecidable, it does not tell us whether
these are r.e. or co-r.e. Indeed we do not have an answer yet to this
question as well for all $\sigma$. For the case of $\sigma = \Sigma$,
the $\ebsSS$ class has a syntactic characterization in the form of
$\bsrS$. Then as seen in section \ref{section:ebs_and_bsr}, $\ebsSS$
is r.e. and not co-r.e. If likewise, for the other $\sigma$'s too, we
can find a syntactic characterization for them or in general a
characterization in terms of any recursive class of formulae, then we
know that they also would be r.e. and not co-r.e.






==> edp.tex <==
\section{A Syntactic sub-class of  $\ebsSs$}\label{section:edp}

$\bsrS$ gave a good starting point as a syntactic
characterization of $\ebsSS$. In this section, we
attempt to provide a syntactic characterization of a fragment of the
$\ebsSs$ class.  Without loss of generality, let $\varphi$ be an
$\FOS$ sentence in prenex conjunctive normal form (PCNF). As
usual, we consider $\Sigma$ as a relational vocabulary. Let
$V(\varphi)$, $EV(\varphi)$ and $AV(\varphi)$ denote respectively the
set of the leftmost existential, non-leftmost (or `inner') existential
and universal variables of $\varphi$. We introduce the following
classification of predicates and their arguments in $\varphi$.
\begin{enumerate}
\item The $i^{th}$ argument (call it $x$) of an instance of predicate
$P$ in $\varphi$ is called (a) \ti{free} if $x \in V(\varphi)$ (b)
\ti{universal} if $x \in AV(\varphi)$, and (c) \ti{existential} if $x
\in EV(\varphi)$.

\item The \emph{free support set} of an instance $I$ of $P$ in
$\varphi$ is the set of all variables in $V(\varphi)$ that appear as
arguments of $I$.  Likewise, the \emph{existential and universal
support sets} of an instance $I$ of $P$ in $\varphi$ are the sets of
variables in $EV(\varphi)$ and $AV(\varphi)$ respectively that appear
as arguments of $I$.

\item An instance $I$ of predicate $P$ in $\varphi$ is called (a)
\ti{free} if its existential and universal support sets are both
empty, (b) \ti{universal} if its existential support set is empty and
universal support set is non-empty, and (c) \ti{existential}
otherwise, i.e., if its existential support set is non-empty.  Note
that an existential instance of $P$ may have a universal argument.

\item Predicate $P$ in $\varphi$ is called (a) \ti{free} if every
instance of $P$ in $\varphi$ is free, (b) \ti{universal} if every
instance of $P$ in $\varphi$ is either universal or free and atleast
one instance is universal, (c) \ti{existential} if atleast one
instance of $P$ in $\varphi$ is existential. Note that an existential
predicate may have a universal or free instance.

\item Two instances of predicate $P$ in $\varphi$ are said to be
\emph{existentially distinguishable} with respect to variable $v$ if
there is an integer $i$ such that (i) the $i^{th}$ argument of each
instance is either free or existential (i.e. not universal) and (ii)
$v$ appears as the $i^{th}$ argument of one instance but not as the
$i^{th}$ argument of the other instance (thus $v \in EV(\varphi) \cup
V(\varphi)$).

\item An instance $I$ of a predicate $P$ is said to have $+ve$
polarity in $\varphi$ (or $I$ is $+ve$ in $\varphi$) if it appears
un-negated in $\varphi$. It is said to have $-ve$ polarity in
$\varphi$ (or $I$ is $-ve$ in $\varphi$) if it appears negated in
$\varphi$.


\end{enumerate}

As an example, consider the sentence
\begin{tabular}{ll}
$\varphi = \exists y \exists u \forall v \exists w$ & $( P(y, y) \vee
\neg Q(u, y) \vee R(y, v)) \wedge$\\
& $( Q(v, u) \vee P(y, u) \wedge \neg R(w, v)))$\\
\end{tabular}
  

Here $ V(\varphi) = \{ y, u\}, AV(\varphi) = \{v\}$ and $EV(\varphi) =
\{w\}$.  For $P$, the free, universal and existential support sets of
the first instance are $\{y\}, \emptyset$ and $\emptyset$
respectively, while those of the second instance are $\{y, u\},
\emptyset$ and $\emptyset$ respectively. Both instances are free and
hence predicate $P$ is free. The first instance of $Q$ is free while
the second instance is universal as its universal support set is $\{ v
\} \neq \emptyset$ and its existential support set is
$\emptyset$. Hence $Q$ is universal. The first instance of $R$ is
universal while its second instance is existential since its
existential support set is $\{w\} \neq \emptyset$. Hence $R$ is
existential. Also the two instances of $R$ are existentially
distinguishable w.r.t. $w$ since (i) the first argument of each
instance is not universal and (ii) $w$ appears as the first argument
of the second instance but not as the first argument of the first
instance. Finally, the first instance of $R$ is $+ve$ i.e. has $+ve$
polarity while the second instance of $R$ is $-ve$ i.e. has $-ve$
polarity in $\varphi$.

Let $\mathsf{U}$ denote the set of all unary predicates of
$\Sigma$. Let $\mc{F}, \mc{A}$ denote respectively the set of all free
and universal predicates of $\Sigma$. Let $E_{\mathsf{U}}$ denote the
set of all variables in $EV(\varphi)$ which appear in $\varphi$ as the
argument of some unary predicate. Let $\overline{E_{\mathsf{U}}} =
EV(\varphi) \setminus E_{\mathsf{U}}$.

\begin{defn}[The $\edpSs$ class]\label{def:edp}
Let $\varphi$ be a $\FOS$ sentence in PCNF. Then $\varphi$ is
said to have \tbf{Existentially Distinguishable Predicates} preserving
$\sigma \subseteq \Sigma$ if the following hold:
\begin{enumerate}
\item $\sigma \subseteq \mathsf{U} \cup \mc{F} \cup \mc{A}$
 \label{edp:cond1}
\item Equality (if present) $\in \mc{F} \cup \mc{A}$.\label{edp:cond2}
\item For any existential predicate $P$ of arity $\geq 2$, every pair
  of instances of $P$ appearing in $\varphi$ in different clauses and
  with different polarities, must be existentially distinguishable
  with respect to atleast one existential variable outside
  $E_{\mathsf{U}}$.\label{edp:cond3}
\end{enumerate}

The set of all $\FOS$ sentences having existentially distinguishable
predicates preserving $\sigma$ is called the $\edpSs$ class.
\end{defn}

Note that a unary predicate or a predicate with arity $\ge 2$ that is
free or universal in $\varphi$ can be either in $\sigma$ or in $\Sigma
\setminus \sigma$.  As an example, consider the sentence
\begin{tabular}{ll}
$\varphi =$ & $ \exists x \exists y \forall z \exists v ((P(x, z) \vee
R(y, z)) \wedge$\\
& $ (\neg P(v, y) \vee P(z, y)) \wedge (\neg R(x, z) \vee (z = x)))$\\
\end{tabular}

Here, $\Sigma = \{P, R\}$, $\mathsf{U} = \mc{F} = \emptyset$, $\mc{A}
= \{R, =\}$ and $E_{\mathsf{U}} = \emptyset$. Consider $\sigma
\subseteq \Sigma$ such that $P \notin \sigma$. Then we can see that
conditions \ref{edp:cond1} and \ref{edp:cond2} in the $\mathbf{EDP}$
definition are satisfied.  Predicate $P$ is existential as its second
instance $P(v, y)$ is existential. For the first and second instances
of $P$ from the left, the second instance is existential and lies in a
different clause and with different polarity w.r.t. the first
instance. Indeed then $v \notin E_{\mathsf{U}}$ existentially
distinguishes the two instances. The second and third instances of $P$
have different polarities but lie in the same clause. The first and
third instances of $P$ lie in different clauses but have the same
polarity. Then these pairs trivially satisfy condition \ref{edp:cond3}
of the $\mathbf{EDP}$ definition. Hence $\varphi \in \edpSs$.

If $P \in \sigma$, then $\varphi \notin
\edpSs$ for any such $\sigma$. This is because $P$
is existential and condition~\ref{edp:cond1} in
Definition~\ref{def:edp} allows only free or universal predicates with
arity $\ge 2$ to be in $\sigma$.

As a second example, consider

\begin{tabular}{ll}
$\psi = $ & $ \exists x \forall z \exists v (P(v, z) \vee Q(z)) \wedge
(P(x, v) \vee \neg Q(v))$ \\
\end{tabular}

Here, $\Sigma = \{P, Q\}$, $\mc{F} = \mc{A} = \{\}, \mathsf{U} = \{Q
\}$. Both $P$ and $Q$ have two instances in different clauses and for
each of $P$ and $Q$, one of its instances is existential. But for $P$,
both its instances are of the same polarity. For $Q$, we find that its
instances even have opposite polarities, but $Q$ is unary. Then both
$P$ and $Q$ satisfy condition \ref{edp:cond3} of Definition
\ref{def:edp} trivially. Hence $\psi(x) \in \edpS{\{Q\}}$ and $\psi(x)
\notin \edpSS$.

\begin{lemma}\label{lemma:edp-simple}
Let $\varphi$ be a $\FOS$ sentence in PCNF in which
\begin{enumerate}
\item For every existential predicate $P$ of arity $\geq 2$ in
$\Sigma$, either (a) all instances of $P$ in $\varphi$ have the same
polarity or (b) all instances of $P$ appear in a single clause.
\item The equality predicate, if present, has free or universal
arguments in all its instances.
\end{enumerate} 
Then there exists $\sigma \subseteq \Sigma$ such that $\varphi \in
\edpSs$.
\end{lemma}

\noindent \emph{Proof:} Let $\sigma \subseteq \Sigma$ be the (possibly
empty) set of unary predicates alongwith the predicates of arity $\ge
2$ that are either free or universal in $\varphi$. Then it easily
follows from Definition~\ref{def:edp} that $\varphi \in
\edpSs$.


\input{edp_subsumed_by_ebs}

\input{ieee_more_on_edp}



==> edp_subsumed_by_ebs.tex <==
\subsection{The $\edpSs$ class as a syntactic
  fragment of the $\ebsSs$ class}
  \label{subsection:proof_that_edp_is_a_frag_of_ebs}

\begin{theorem}\label{thm:edp-bound}
Let $\varphi$ be a $\FOS$ sentence in $\edpSs$. Let $k$ be the number
of unary predicates in $\Sigma$. Then $\varphi$ satisfies all
conditions in Definition~\ref{def:ebs_general} (of section
\ref{section:ebs_sigma_introduction}) with $\mc{B} = |V(\varphi)| +
|\overline{E_{\mathsf{U}}}| + 2^k$.
\end{theorem}

Before proving this result, we see that this theorem immediately
implies the following.

\begin{Corollary}\label{cor:edp-ebs}
  $\forall \sigma \subseteq \Sigma$, $\edpSs
\subseteq \ebsSs$.
\end{Corollary}

Thus $\edpSs$ is a syntactic fragment of $\ebsSs$. We shall explore
the quesrion of whether $\edpSs$ is a syntactic characterization of
$\ebsSs$ in the forthcoming sections. We now present the proof of
Theorem \ref{thm:edp-bound}. The proof is a bit long so while the
interested reader is urged to go through it, the proof if skipped
would not affect the flow.


\subsubsection{Proving Theorem \ref{thm:edp-bound}}

We prove a stronger version of Theorem \ref{thm:edp-bound} namely for
formulae with free variables. The results naturally follows for
sentences too. 

For the case of free variables, the $\mathbf{EBS}$ definition is slightly
widened to also assert that if $M \models \varphi(\tbf{a})$ where
$\tbf{a}$ is a vector of elements from $M$, then $M_1$ must contain
\tbf{a}. The other conditions remain exactly the same.\\

Our proof is motivated by the proof of finite model size of formulae
in the L\"owenheim class and the Bernays-Sch\"onfinkel-Ramsey class,
as given in~\cite{BGG}.

Consider a $\Sigma-$structure $M$ with universe $\mc{U}_M$ and
$\tbf{a} \in \mc{U}_M^{|\tbf{x}|}$ such that $M \models
\varphi(\tbf{a})$ and $|\mc{U}_M| > m + |V(\varphi(\tbf{x}))| +
|\overline{E_{\mathsf{U}}}| + 2^k$.

Now we have that $|\mc{C}| = m$ and $|\mathsf{U}| = k$.  Let $A'
\subseteq \mc{U}_M$ be the set of interpretations of the constants of
$\mc{C}$ in the model $M$.  Let $A'' \subseteq \mc{U}_M$ be the set of
values assigned to variables in $V(\varphi(\tbf{x}))$ in showing that
$M \models \varphi(\tbf{a})$ (The existential variables in
$EV(\varphi(\tbf{x}))$ being the leftmost, the values assigned to them
in $M$ are independent of the values of all the universal variables).
Thus, $A''$ contains all values in $\tbf{a}$ and also values assigned
to variables bound to the leftmost existential quantifiers in
$\varphi(\tbf{x})$.  Clearly, $ |A'| \leq m$ and $|A''| \leq
|V(\varphi(\tbf{x}))|$. Since as per our terminology, all the
arguments belonging to $V(\varphi(\tbf{x})) \cup \mc{C}$ are called
\ti{free} arguments, we denote by $\ti{Free}$ the set
$V(\varphi(\tbf{x})) \cup \mc{C}$ and by $\tbf{Val}(\ti{Free})$ the
set of values in $M$, for the elements of \ti{Free} i.e.
$\tbf{Val}(\ti{Free}) = A' \cup A''$.\\


Without loss of generality, let $\mathsf{U} = \{Q_1, \ldots, Q_k\}$.
For every element $e$ in the universe $\mc{U}_M$, we associate a
binary vector or \emph{colour} $C(e) \in \{0,1\}^k$, where the
$i^{th}$ component of $C(e)$ is $1$ iff $M \models Q_i(e)$.  For every
$c \in \{0,1\}^k$, let $\mc{U}_{M}^c$ denote the subset of elements of
$\mc{U}_M$ that have the colour $c$. 

Consider the set $\mc{V}_M^c = \mc{U}_M^c \setminus
\tbf{Val}(\ti{Free})$. We now choose a subset $A^c$ of $\mc{V}_{M}^c$
as follows: if $\mc{V}_{M}^c = \emptyset$, then $A^c = \mc{V}_{M}^c =
\emptyset$; otherwise, $A^c$ is a singleton set formed by selecting
any element $a^c$ from $\mc{V}_{M}^c$ (i.e. $A^c = \{ a^c \}$).

Let $\overline{E_{\mathsf{U}}} = EV(\varphi(\tbf{x})) \setminus
E_{\mathsf{U}}$ denote the complement of $E_{\mathsf{U}}$ within
$EV(\varphi(\tbf{x}))$. $\overline{E_{\mathsf{U}}}$ denotes the set of
all variables of $EV(\varphi(\tbf{x}))$ that do not appear in
$\varphi(\tbf{x})$ as an argument of any instance of any unary
predicate. Then we finally choose a subset of $\mc{U}_M$ of size
$|\overline{E_{\mathsf{U}}}|$ which we denote as
$\tbf{Val}(\overline{E_{\mathsf{U}}})$ such that (i)
$\tbf{Val}(\overline{E_{\mathsf{U}}}) \bigcap \tbf{Val}(\ti{Free}) =
\emptyset$ and (ii) $\tbf{Val}(\overline{E_{\mathsf{U}}}) \bigcap A^c
= \emptyset$ for all colours $c \in \{0, 1\}^k$.

Note that
\begin{eqnarray}
& |\tbf{Val}(\ti{Free})| + |\tbf{Val}(\overline{E_{\mathsf{U}}})| +
\Sigma_{c \in \{0, 1\}^k} |A^c| \nonumber\\ 
\leq & |A'| + |A''| + |\overline{E_{\mathsf{U}}}| + 
\Sigma_{c \in \{0, 1\}^k} 1 \nonumber\\
\leq & m + |V(\varphi(\tbf{x}))| + |\overline{E_{\mathsf{U}}}| +
2^k \nonumber \\ 
\nonumber
\end{eqnarray}

so that we can indeed choose the subset
$\tbf{Val}(\overline{E_{\mathsf{U}}})$ of $\mc{U}_M$ of the mentioned
size. We denote the elements of $\tbf{Val}(\overline{E_{\mathsf{U}}})$
as $a_i$ where $i$ is such that $v_i \in \overline{E_{\mathsf{U}}}$
(thus $\tbf{Val}(\overline{E_{\mathsf{U}}}) = \{ a_i | v_i \in
\overline{E_{\mathsf{U}}}\}$). Note that the sets
$\tbf{Val}(\ti{Free})$, $\tbf{Val}(\overline{E_{\mathsf{U}}})$ and
$A^c$ are all disjoint with each other for each $c \in \{0,
1\}^k$. Further $A^{c_1}$ and $A^{c_2}$ are also disjoint with each
other for all $c_1, c_2 \in \{0, 1\}^k$ where $c_1 \neq c_2$.\\

We now consider the sub-structure $M_1$ of $M$ generated by
$\tbf{Val}(\ti{Free}) \cup \tbf{Val}(\overline{E_{\mathsf{U}}}) \cup
\bigcup_{c \in \{0, 1\}^k} A^c$. We show that this sub-structure $M_1$ 
satisfies all of the $\mathbf{EBS}$ conditions with $\mc{B} = m +
|V(\varphi(\tbf{x}))| + |\overline{E_{\mathsf{U}}}| + 2^k$. 


Since $\varphi(\tbf{x})$ is in prenex normal form, we assume without
loss of generality that

\begin{tabular}{lll}
$\varphi(\tbf{x})$ & = & $\exists
\tbf{v}_{\textrm{\scriptsize{\ti{leftmost}}}}
\forall \tbf{z}_0 \exists v_1 \forall \tbf{z}_1 \exists v_2 
\forall \tbf{z}_2 \ldots \exists v_r \forall \tbf{z}_r$\\
& & $\psi(\tbf{x}, \tbf{v}_{\textrm{\scriptsize{\ti{leftmost}}}}, \tbf{z}_0, 
v_1, \tbf{z}_1, \ldots v_r, \tbf{z}_r)$\\
\end{tabular}

where $\psi$ is a quantifier-free matrix in CNF,
$\tbf{v}_{\textrm{\scriptsize{\ti{leftmost}}}}$ denotes the (possibly empty)
set of variables bound to the leftmost quantifiers (all of these
variables are thus in $V(\varphi(\tbf{x}))$), $r$ denotes
$|EV(\varphi(\tbf{x}))|$ and $\tbf{z}_i$ denotes the (possibly empty)
vector of universally quantified variables that appear immediately to
the right of the existentially quantified variable $v_i$ in the
quantifier prefix of $\varphi(\tbf{x})$. Let $\tbf{z} = (\tbf{z}_0,
\tbf{z}_1, \ldots, \tbf{z}_r)$ denote the tuple of all the
$AV(\varphi(\tbf{x}))$ variables and $\tbf{v} = (v_1, v_2, \linebreak
\ldots, v_r)$ denote the tuple of all the $EV(\varphi(\tbf{x}))$
variables. For every extension $M_2$ of $M_1$ within $M$, we now
describe how to construct a $\Sigma-$structure $M_2'$ such that
$\mc{U}_{M_2} = \mc{U}_{M_2'}$, $M_2' \models \varphi(\tbf{a})$ and
$M_2'|_{\sigma} = M_2|_{\sigma}$.\\

If $M_2 \models \varphi(\tbf{a})$, we simply choose $M_2' = M_2$.
Clearly, this choice satisfies the $\mathbf{EBS}$ conditions.  If $M_2
\not\models \varphi(\tbf{a})$, we must redefine the interpretations of
(some) predicates in $\Sigma \setminus \sigma$ such that the resulting
structure $M_2'$ is a model of $\varphi(\tbf{a})$. We note that this
$M_2'$ has the same universe namely $\mc{U}_{M_2}$ as $M$
i.e. $\mc{U}_{M_2'} = \mc{U}_{M_2}$. Therefore henceforth we will
refer to the universe of $M_2'$ as $\mc{U}_{M_2}$.\\


The way we proceed is we first create a \ti{quasi} $\Sigma-$structure
$M_3$ which has the universe $\mc{U}_{M_2}$ and such that
$\varphi(\tbf{a})$ is $\mathsf{True}$ in it. It is \ti{quasi} in the
sense that it gives \ti{atleast} one truth value to each predicate of
$\Sigma$ for each valuation of its arguments. In other words, it could
give both truth values to a predicate for certain valuations of its
arguments. The desired $M_2'$ would then be extracted out from this
quasi $\Sigma-$structure $M_3$.

In the following, we overload the $\models$ symbol so that we denote
$\varphi(\tbf{a})$ being $\mathsf{True}$ in $M_3$ as $M_3 \models
\varphi(\tbf{a})$.

Now, in order to get $M_3$, we observe that for every assignment of
values $\tbf{Z}$ from $\mc{U}_{M_2}$ to the universally quantified
variables $\tbf{z}$ in $\varphi(\tbf{a})$, we must choose a value from
$\mc{U}_{M_2}$ for each of the constants in $\mc{C}$ and each of the
existentially quantified variables, namely the variables in
$\tbf{v}_{\textrm{\scriptsize{\ti{leftmost}}}}$ and those in
$\tbf{v}$, such that $\psi(\tbf{x},
\tbf{v}_{\textrm{\scriptsize{\ti{leftmost}}}}, \tbf{z}_0, v_1,
\tbf{z}_1, \ldots v_r, \tbf{z}_r)$ instantiated with these values
evaluates to $\mathsf{True}$ in $M_3$. Suppose we are indeed able to
choose these values from $\mc{U}_{M_2}$. Upon substitution of these
values in $\psi$, call the resulting fully instantiated matrix as
$\psi_{M_3}[\tbf{Z}]$ (Note the square brackets in the notation which
are used to mean that $\tbf{Z}$ is considered as an `input' to give as
`output', a fully instantiated matrix denoted as
$\psi_{M_3}[\tbf{Z}]$. It should \ti{not} be looked at as meaning that
$\psi_{M_3}$ is a formula whose free variables are being instantiated
with $\tbf{Z}$ - in that case we would use round brackets around
$\tbf{Z}$).


Before proceeding ahead, we observe that there are two tasks to be
done. The first is, given a valuation $\tbf{Z}$ of the universal
variables, choosing the values for the constants and all the
existential variables to substitute in $\psi$ to get
$\psi_{M_3}[\tbf{Z}]$. The second is to define the (quasi) structure
$M_3$ over which $\psi_{M_3}[\tbf{Z}]$ evaluates to $\mathsf{True}$
for each valuation $\tbf{Z}$ from $\mc{U}_{M_2}$ of the $\tbf{z}$
variables so that as a result $M_3 \models \varphi(\tbf{a})$.

For the first task, we choose the values as follows:
\begin{enumerate}
\item For each constant in $\mc{C}$, we interpret it in $M_3$ with the
same value with which it is interpreted in $M$. Likewise for each
variable of $V(\varphi((\tbf{x}))$, we substitute for it the same
value which is assigned to it in $M$ (This is possible since
$\tbf{Val}(\ti{Free}) \subseteq \mc{U}_{M_2}$). These values of course
are independent of the instantiations $\tbf{Z}$ for the $\tbf{z}$
variables. This takes care of all elements of \ti{Free}.
\item 
For each variable $v_i \in \overline{E_{\mathsf{U}}}$, we assign it
the value $a_i \in \tbf{Val}(\overline{E_{\mathsf{U}}}) \subseteq
\mc{U}_{M_2}$. These values too are independent of the instantiations
of the $\tbf{z}$ variables.
\item 
Given a valuation $\tbf{Z}$ of the $\tbf{z}$ variables, for each
variable $v_i \in E_{\mathsf{U}}$, we do the following.  We turn to
the model $M$ and look at the assignment made to the $\tbf{v}$
variables in $\psi$ for this valuation, namely \tbf{Z}, of the
$\tbf{z}$ variables. Since $M \models \varphi(\tbf{a})$, we know that
there exists a choice of values from $\mc{U}_M$ for each existentially
quantified variable and the constants such that when these values are
substituted in $\psi(\tbf{x},
\tbf{v}_{\textrm{\scriptsize{\ti{leftmost}}}},
\tbf{z}_0, v_1, \tbf{z}_1, \ldots ~~ v_r, \tbf{z}_r)$, we get a fully
instantiated matrix - which we denote as $\psi_M[\tbf{Z}]$ - which
evaluates to $\mathsf{True}$ in $M$. Let $d$ be the value substituted
for $v_i$ from $\mc{U}_M$ in making $\psi_M[\tbf{Z}]$ $\mathsf{True}$
in $M$. Let $c$ be the colour of $d$ in $M$.
\begin {enumerate}
\item 
If $d$ belongs to $\tbf{Val}(\ti{Free})$, then we choose the same
value $d$ to substitute for $v_i$ from $\mc{U}_{M_2}$ (This is
possible because $\tbf{Val}(\ti{Free}) \subseteq \mc{U}_{M_2}$).
\item 
If $d$ is not in $\tbf{Val}(\ti{Free})$, then we choose the value $a^c \in A^c
\subseteq \mc{U}_{M_2}$ to substitute for $v_i$.
\end{enumerate}
\end{enumerate}

Using the above procedure (call it \ti{Selector}), for each valuation
$\tbf{Z}$ of the $\tbf{z}$ variables, we determine the values to
assign to each of the existential variables and constants and
substituting all these values in $\psi$, we get the fully
instantitated matrix $\psi_{M_3}[\tbf{Z}]$.

We now take up the second task namely defining $M_3$ such
that $M_3 \models \varphi(\tbf{a})$.\\

Before proceeding ahead, we introduce a little terminology to make
further explanations easier. If $I$ denotes the instance of a
predicate $P$ in $\psi$, we denote by $I_{M}[\tbf{Z}]$, the instance
$I$ as it appears in $\psi_{M}[\tbf{Z}]$ (Thus $I_M[\tbf{Z}]$ would
look like $P(\tbf{d})$ where the values in $\tbf{d}$ come from
$\mc{U}_M$). Likewise we denote by $I_{M_3}[\tbf{Z}]$, the instance
$I$ as it appears in $\psi_{M_3}[\tbf{Z}]$.

Then for each valuation $\tbf{Z}$ of the $\tbf{z}$ variables, for each
predicate $P \in \Sigma \cup \{ = \}$ and for each instance $I$ of $P$
in $\psi$, we do the following:
\begin{enumerate}
\item 
If $P$ is nullary (i.e. constant), then we have already stated above
how $P$ must be interpreted in $M_3$.
\item 
If $P \in \mathsf{U}$, then $I_{M_3}[\tbf{Z}]$ is assigned the same
truth value in $M_3$ as $I_M[\tbf{Z}]$ has in $M$. In other words
$M_3 \models I_{M_3}[\tbf{Z}]$ iff $M \models I_M[\tbf{Z}]$.
\item 
If $P$ is atleast 2-ary, we have the following:
\begin{enumerate}
\item If $P$ is a free or universal predicate, then $I_{M_3}[\tbf{Z}]$
is assigned a truth value such that $M_3 \models I_{M_3}[\tbf{Z}]$ iff $M
\models I_M[\tbf{Z}]$.
\item If $P$ is an existential predicate, then $I_{M_3}[\tbf{Z}]$ is
assigned a truth value such that
\begin{itemize}
\item 
$M_3 \models I_{M_3}[\tbf{Z}]$ if $I$ is $+ve$ in $\psi$ and
\item
$M_3 \models \neg I_{M_3}[\tbf{Z}]$ if $I$ is $-ve$ in $\psi$.
\end{itemize}
\end{enumerate}
\end{enumerate}

By the above, for each valuation $\tbf{Z}$ of $\tbf{z}$, since either
we have given an instance in $\psi_{M_3}[\tbf{Z}]$ the same truth
value in $M_3$ as the corresponding instance in $\psi_M[\tbf{Z}]$ has
in $M$ or we have made the literal corresponding to the instance
$\mathsf{True}$ in $M_3$, we can see that $\psi_{M_3}[\tbf{Z}]$ is
true in $M_3$ since $\psi_M[\tbf{Z}]$ is true in $M$.

We note now that by the above procedure, we would have
\ti{interpreted} in $M_3$ (i.e. given truth values in $M_3$ to) all
the predicates in $\Sigma$ for those values of their arguments which
were seen in the `$\psi_{M_3}[\tbf{Z}]$'s that were obtained when
enlisting all the valuations $\tbf{Z}$ of the universally quantified
variables. Lets call this whole procedure as procedure $\mc{P}_1$.

In general, $\mc{P}_1$ might not exhaust all possible argument values
for all the predicates and hence the interpretation of the predicates
in $M_3$ would be partial and incomplete. In order to give the
complete interpretation in $M_3$ for each predicate in $\Sigma$, we
need to consider for each predicate, those values for its arguments
that were not covered by $\mc{P}_1$. As for the interpretations of the
predicates for these values (i.e. which were not covered by
$\mc{P}_1$), it doesnt matter in which way they are interpreted
because these values do not in any way contribute towards making
$\psi_{M_3}[\tbf{Z}] ~~\mathsf{True}$ in $M_3$ for any valuation
$\tbf{Z}$ from $\mc{U}_{M_2}$ of the $\tbf{z}$ variables (and hence in
showing $M_3 \models \varphi(\tbf{a})$). Hence, in particular, they
could be interpreted as they are in $M$. Lets call this procedure of
assignment of truth values to the predicates of $\Sigma$ for their
remaining argument values as procedure $\mc{P}_2$. Clearly procedures
$\mc{P}_1$ and $\mc{P}_2$ completely define in $M_3$, the
interpretations of all predicates for all values of their
arguments. Further they define interpretations of the predicates for
disjoint sets of values of their arguments.\\

Having defined $M_3$, we now see that it is possible that above
procedures $\mc{P}_1$ and $\mc{P}_2$ together give interpretations to
the predicates of $\Sigma$ in $M_3$ that cause a \ti{conflict} i.e. a
predicate being assigned both $\mathsf{True}$ and $\mathsf{False}$
values in $M_3$ for the same values of its arguments. Conflicts thus
make $M_3$ a quasi $\Sigma-$structure (and not a
$\Sigma-$structure). In what follows we show that either conflicts are
\ti{prevented} by the $\mathbf{EDP}$ conditions or conflicts that are not
prevented can be \ti{cured} (resolved) without affecting the truth of
$\varphi(\tbf{a})$ in the `cured' $M_3$. In other words, we will be
able to construct the desired model $M_2'$ by simply curing all the
conflicts in $M_3$ (i.e. by extracting the appropriate truth value in
case of a conflict). Then $M_2'$ would be a valid $\Sigma-$structure
giving unique truth values to each predicate for each valuation of its
arguments. Further $M_2'$ would be a model for $\varphi(\tbf{a})$
i.e. $M_2' \models \varphi(\tbf{a})$.

Before going ahead, we note that $M$ is clearly free of any
conflicts.\\

\underline{\tbf{Handling conflicts}}\\\\ 
Suppose there was a conflict i.e. a predicate $P$ got assigned both
$\mathsf{True}$ and $\mathsf{False}$ values in $M_3$ for the same
vector of values (say $\tbf{d}$) as its argument. Then we have the
following cases:
 
1) Suppose the two different truth values to $P(\tbf{d})$ are both
assigned by $\mc{P}_2$. But $\mc{P}_2$ assigns the same truth values
as in $M$. This shows that there must be a conflict in $M$ itself
which we know is not the case.
 
2) Without loss of generality, suppose $P(\tbf{d})$ is assigned
$\mathsf{True}$ by $\mc{P}_1$ and $\mathsf{False}$ by $\mc{P}_2$. Then
as seen above, since $\mc{P}_1$ and $\mc{P}_2$ give truth values for
disjoint sets of values of arguments, $P(\tbf{d})$ would be assigned a
truth value either only by $\mc{P}_1$ or only by $\mc{P}_2$
contradicting the assumption above.
 
3) $P(\tbf{d})$ is assigned both the truth values by $\mc{P}_1$. We
abbreviate the truth value $\mathsf{True}$ as $t$ and $\mathsf{False}$
as $f$. Having seen how the procedure $\mc{P}_1$ works, we conclude
that for each truth value $\alpha \in \{ t, f \}$, $P(\tbf{d})$ must
then have appeared in $\psi_{M_3}[\tbf{Z}_{\alpha}]$ for some
valuation $\tbf{Z}_\alpha$ of the \tbf{z} variables where it was
assigned that truth value (namely $\alpha$). Let for truth value
$\alpha$, the instance $I^\alpha$ of $P$ in $\psi$ be instantiated in
$\psi_{M_3}[\tbf{Z}_{\alpha}]$ to get $P(\tbf{d})$. In particular, the
instance $I^t$ of $P$ in $\psi$ gets instantiated in
$\psi_{M_3}[\tbf{Z}_t]$ to get $P(\tbf{d})$ and the instance $I^f$ of
$P$ in $\psi$ gets instantiated in $\psi_{M_3}[\tbf{Z}_f]$ to get
$P(\tbf{d})$.

Using our notation introduced earlier, the instances mentioned above
would be denoted as $I^t_{M_3}[\tbf{Z}_t]$ and
$I^f_{M_3}[\tbf{Z}_f]$ respectively ($I^t_{M_3}[\tbf{Z}_t] ~= ~
I^f_{M_3}[\tbf{Z}_f] ~=~ P(\tbf{d})$).  Further the former instance
is assigned truth value as $\mathsf{True}$ and the latter is assigned
$\mathsf{False}$ in $M_3$.


Before proceeding ahead, we make the following observation.


\begin{lemma}\label{proof-helper-1}
Consider an instance $I$ in $\psi$ of a predicate $P$. Let $\tbf{Z}$
be an instantiation from $\mc{U}_{M_2}$, of all the universal
variables $\tbf{z}$. Then the following are true:
\begin{enumerate}
\item 
For each $i$ ranging from 1 to the arity of $P$, if either (i) the
$i^{th}$ argument of $I$ in $\psi$ is universal or (ii) the $i^{th}$
argument of $I_{M_3}[\tbf{Z}]$ is from $\tbf{Val}(\ti{Free})$, then
the $i^{th}$ argument of $I_{M}[\tbf{Z}]$ is the same as the $i^{th}$
argument of $I_{M_3}[\tbf{Z}]$. \label{proof-helper-1-1}

\item 
If $I$ is a free or a universal instance in $\psi$, then
$I_{M}[\tbf{Z}]$ and $I_{M_3}[\tbf{Z}]$ have the same vector of
values appearing as their arguments. \label{proof-helper-1-2}

\end{enumerate}
\end{lemma}

\ti{Proof:}
\begin{enumerate}
\item 
(i) If the $i^{th}$ argument is universal, then since
  $\psi_{M_3}[\tbf{Z}]$ and $\psi_{M}[\tbf{Z}]$ have the same
  valuation of all the universal variables, namely \tbf{Z}, then in
  particular for the $i^{th}$ argument of $I$, the same value is
  substituted for it in both $\psi_{M_3}[\tbf{Z}]$ and
  $\psi_{M}[\tbf{Z}]$.

(ii) If the $i^{th}$ argument of $I_{M_3}[\tbf{Z}]$ is from
  $\tbf{Val}(\ti{Free})$, then it means that the $i^{th}$ argument of
  $I$ is either (a) free or (b) universal or (c) a variable in
  $E_{\mathsf{U}}$. For (a) and (c), we see directly from cases (1)
  and (3a) of \ti{Selector} that the $i^{th}$ argument of
  $I_{M}[\tbf{Z}]$ is the same as the $i^{th}$ argument of
  $I_{M_3}[\tbf{Z}]$. For (b), the reasoning is already presented
  above.

\item
If $I$ is a free or a universal instance, each argument of it is
either free or universal. Then by applying the reasoning presented in
the preceding point to all arguments $i$ ranging from 1 to the arity
of $P$, we can see that $I_{M}[\tbf{Z}]$ and $I_{M_3}[\tbf{Z}]$ will
have the same vector of values appearing as their arguments. 

\end{enumerate}
\epf

Coming back to checking for conflicts, we have the following
possibilities:

\begin{enumerate}
\item $P$ is unary. Then $\tbf{d} = d$ (say).

(a) If $I^t$ and $I^f$ are free or universal instances, then from
Lemma \ref{proof-helper-1}(2), for each truth value $\alpha \in \{t,
f\}$, $I^{\alpha}_{M}[\tbf{Z}_{\alpha}]$ and
$I^{\alpha}_{M_3}[\tbf{Z}_{\alpha}]$ have the same value as their
argument (namely $d$). Then $I^t_{M}[\tbf{Z}_t] = I^f_{M}[\tbf{Z}_f] =
P(d)$.

(b) If $d \in \tbf{Val}(\ti{Free})$, then from Lemma
\ref{proof-helper-1}(1), we again see similarly that
$I^t_{M}[\tbf{Z}_t] = I^f_{M}[\tbf{Z}_f] = P(d)$.

In either of the above cases, from case (2) of $\mc{P}_1$,
$I^{\alpha}_{M}[\tbf{Z}_{\alpha}]$ and
$I^{\alpha}_{M_3}[\tbf{Z}_{\alpha}]$ have the same truth value (namely
$\alpha$) in $M$ and $M_3$ respectively. But then this shows that
$P(d)$ is assigned both truth values in $M$ thus showing a conflict in
$M$ itself which we know does not exist.

Without loss of generality, suppose $I^t$ is an existential instance
(i.e. of the form $P(v)$ where $v \in EV(\varphi(\tbf{x}))$). Note
that the argument $v$ cannot belong to
$\overline{E_{\mathsf{U}}}$. The case when $v$ is assigned the value
$d \in \tbf{Val}(\ti{Free})$ is already considered above. Then from
case 3(b) of \ti{Selector}, the only remaining case is when $d = a^c$
for some colour $c$. Since $a^c$ appears as the argument of
$I^t_{M_3}[\tbf{Z}_t]$, from case (3b) of \ti{Selector}, it means that
the colour of $a^c$ in $M$ is $c$. If $I^t_{M}[\tbf{Z}_t] = P(d_1)$,
then the colour of $d_1$ is also $c$. Further since by case(2) of
$\mc{P}_1$, $M \models I^t_{M}[\tbf{Z}_t]$ iff $M_3 \models
I^t_{M_3}[\tbf{Z}_t]$, we have that $P(d_1)$ is $\mathsf{True}$ in
$M$. Then since both $d_1$ and $a^c$ have the same colour in $M$, we
have that $P(a^c)$ is also $\mathsf{True}$ in $M$.

Since the argument of $I^f_{M_3}[\tbf{Z}_f]$ is also $a^c$, it means
that the argument of $I^f$ is either (i) universal or (ii) existential
(in particular, belonging to $E_{\mathsf{U}}$. In case of (i), by
Lemma \ref{proof-helper-1}(2), $I^f_{M}[\tbf{Z}_f] =
I^f_{M_3}[\tbf{Z}_f] = P(a^c)$. By case (2) of $\mc{P}_1$, $M \models
I^f_{M}[\tbf{Z}_f]$ iff $M_3 \models I^f_{M_3}[\tbf{Z}_f]$, so that
$P(a^c)$ is $\mathsf{False}$ in $M$. But this is a contradiction.

In case of (ii), suppose $I^f_{M}[\tbf{Z}_f] = P(d_2)$. Since
$I^f_{M_3}[\tbf{Z}_f] = P(a^c)$, by case (3b) of \ti{Selector}, $d_2$
has the colour $c$. Then $P(d_2)$ is $\mathsf{True}$ in $M$. But by
case (2) of $\mc{P}_1$, $M \models I^f_{M}[\tbf{Z}_f]$ iff $M_3
\models I^f_{M_3}[\tbf{Z}_f]$ so that $P(d_2)$ is $\mathsf{False}$ in
$M$. Now since $d_2$ and $a^c$ have the same colour in $M$, we must
have that $P(a^c)$ is $\mathsf{False}$ in $M$. This is again a
contradiction.

Thus there are no conflicts in $M_3$ as far as the unary predicates
go.

 
\item
$P$ is of arity $\geq 2$ and is a free or universal predicate.

Then each of $I^t$ and $I^f$ is either universal or free in
$\varphi(\tbf{x})$. Then from Lemma \ref{proof-helper-1}(2), for each
truth value $\alpha \in \{t, f\}$, $I^{\alpha}_{M}[\tbf{Z}_{\alpha}]$
and $I^{\alpha}_{M_3}[\tbf{Z}_{\alpha}]$ have the same vector of
values as their arguments (namely $\tbf{d}$). Further by case (3a) of
$\mc{P}_1$, both have the same truth value (namely $\alpha$) in $M$
and $M_3$ respectively. But then this shows that $I^t_{M}[\tbf{Z}_t] =
I^f_{M}[\tbf{Z}_f] = P(\tbf{d})$ and that $P(\tbf{d})$ is assigned
both truth values in $M$ thus showing a conflict in $M$ itself which
we know does not exist.

Thus there are no conflicts in $M_3$ for the free and universal
predicates too.

\item
$P$ is of arity $\geq 2$ and is an existential predicate. 

If $I^t$ and $I^f$ are of the same polarity in $\varphi(\tbf{x})$,
then from case (3b) of $\mc{P}_1$, we see that in $M_3$, both
$I^t_{M_3}[\tbf{Z}_t]$ and $I^f_{M_3}[\tbf{Z}_f]$ have the same truth
value - $\mathsf{True}$ if their polarity is $+ve$ and $\mathsf{False}$
if their polarity is $-ve$. Then there is no conflict in the first
place.

If $I^t$ and $I^f$ are of opposite polarity, then suppose that they
were in different clauses. From the last condition of the $\mathbf{EDP}$
definition, there is a variable $v_l \in \overline{E_{\mathsf{U}}}$
such that $I^t$ and $I^f$ would be existentially distinguishable by
it. Suppose it appears as the $n^{th}$ argument of $I^f$. Then the
$n^{th}$ argument of $I^t$ would be either an variable $v \in
\ti{Free}$ or a variable $v_p \in E_{\mathsf{U}}$ or a variable $v_r
\in \overline{E_{\mathsf{U}}}$ where $r \neq l$. Then \ti{Selector}
would assign the $n^{th}$ argument of $I^f_{M_3}[\tbf{Z}_f]$ as $a_l
\in \tbf{Val}(\overline{E_{\mathsf{U}}})$ while the $n^{th}$ argument
of $I^t_{M_3}[\tbf{Z}_t]$ would be respectively assigned a value
either from (i) $\tbf{Val}(\ti{Free})$ or from (ii) $A^c \neq
\emptyset$ for some colour $c$ or (iii) $a_r \in
\tbf{Val}(\overline{E_{\mathsf{U}}})$. The values in case of (i) and
(ii) must be different from $a_l$ since
$\tbf{Val}(\overline{E_{\mathsf{U}}})$ is disjoint with both
$\tbf{Val}(\ti{Free})$ and $A^c$. In case of (iii), since $r \neq l$,
$a_r \neq a_l$. Thus in all cases, the $n^{th}$ argument of
$I^f_{M_3}[\tbf{Z}_f]$ would be different from that of
$I^t_{M_3}[\tbf{Z}_t]$. Then the conflict couldn't have happened at
all. A similar argument can be given for the case when $v_l$ appears
as the $n^{th}$ argument of $I^t$.

(We thus note how the last condition in the $\mathbf{EDP}$ definition
\ti{prevents} the occurence of a conflict.)


Finally consider the case that $I^t$ and $I^f$ are of opposite
polarity and are in the same clause say $C$ of $\psi$. Then since $M_3
\models I^t_{M_3}[\tbf{Z}_t]$ and $M_3 \models \neg
I^f_{M_3}[\tbf{Z}_f]$, by case (3b) of $\mc{P}_1$, we have that $I^t$
is $+ve$ while $I^f$ is $-ve$ in $\varphi(\tbf{x})$.  Then for the
valuation $\tbf{Z}_f$ of the $\tbf{z}$ variables, $\mc{P}_1$ would
assign $I^t_{M_3}[\tbf{Z}_f]$, the value $\mathsf{True}$ in $M_3$. Let
$C[\tbf{Z}_f]$ be the clause $C$ as it appears in
$\psi_{M_3}[\tbf{Z}_f]$. Then $C[\tbf{Z}_f]$ which contains
$I^t_{M_3}[\tbf{Z}_f]$ and $I^f_{M_3}[\tbf{Z}_f]$, is not dependent on
the literal corresponding to $I^f_{M_3}[\tbf{Z}_f]$ for $C[\tbf{Z}_f]$
to become $\mathsf{True}$ in $M_3$ as $I^t_{M_3}[\tbf{Z}_f]$ is
already $\mathsf{True}$ in $C[\tbf{Z}_f]$. Then we \ti{cure} the
conflict on the value of $P(\tbf{d})$ ($ = I^t_{M_3}[\tbf{Z}_t] =
I^f_{M_3}[\tbf{Z}_f]$) by fixing the value of $P(\tbf{d})$ in $M_3$ to
be $\mathsf{True}$.

Now since $M_3 \models \varphi(\tbf{a})$, we have that for every
clause $C_1$ of $\psi$, $C_1[\tbf{Z}]$ is true in $M_3$ for each
valuation $\tbf{Z}$ of the $\tbf{z}$ variables ($C_1[\tbf{Z}]$ is the
clause $C_1$ as it appears in $\psi_{M_3}[\tbf{Z}]$).  We note that
while the fixing mentioned above doesnt affect the truth of clause
$C[\tbf{Z}_f]$, we now investigate whether this makes some other
clause $\mathsf{False}$ i.e. does there exist a valuation $\tbf{Z}^*$
of $\tbf{z}$ and a clause $C^*$ of $\psi$ such that in
$\psi_{M_3}[\tbf{Z}^*]$, the clause $C^*[\tbf{Z}^*]$ (which is the
clause $C^*$ as it appears in $\psi_{M_3}[\tbf{Z}^*]$) became
$\mathsf{False}$ due to the fixing. Suppose there is such a
$\tbf{Z}^*$. Since the fixing caused the change of truth value of
$C^*[\tbf{Z}^*]$ from $\mathsf{True}$ to $\mathsf{False}$, it must be
the case that there is an instance $I^*$ of $P$ appearing in
$C^*[\tbf{Z}^*]$ such that $I^*_{M_3}[\tbf{Z}^*] = P(\tbf{d})$ and
such that $I^*$ is $-ve$ in $\psi$. Further $I^*_{M_3}[\tbf{Z}^*]$ was
earlier (i.e. before the fixing) assigned value $\mathsf{False}$
(making its corresponding literal $\mathsf{True}$) and every other
literal in $C^*[\tbf{Z}^*]$ is assigned value $\mathsf{False}$.

We firstly note that $I^* \neq I^t$ since they are of opposite
polarities. If $C^* \neq C$, then $I^t$ and $I^*$ are two instances of
$P$ of opposite polarity appearing in different clauses, which had
earlier (i.e. before the fixing) conflicted. But in the analysis shown
above we know that this cannot happen. Then $C^* = C$. But then by
case (3b) of $\mc{P}_1$, $I^t_{M_3}[\tbf{Z}^*]$ would be assigned
$\mathsf{True}$ in $M_3$.  But this contradicts the conclusion made
above that the literal corresponding to $I^*_{M_3}[\tbf{Z}^*]$ was the
only literal in $C^*[\tbf{Z}^*]$ that made the latter $\mathsf{True}$.

Thus, by fixing the value of $P(\tbf{d})$ to $\mathsf{True}$, the
conflict is eliminated and further for every clause $C$ in $\psi$ and
for every valuation $\tbf{Z}$ of $\tbf{z}$, $C[\tbf{Z}]$ continues to
remain $\mathsf{True}$ so that $\varphi(\tbf{a})$ continues to be
$\mathsf{True}$ in the new $M_3$ which is cured of one conflict.

Since $M_3$ is of finite size, there are only a finite number of
conflicts and the curing process above eliminates conflicts one at a
time while still preserving the truth of $\varphi(\tbf{a})$ in the new
$M_3$ obtained after the curing. Then this process terminates, giving
a \ti{fully cured} $M_3$ which we call $M_2'$ such that $M_2'$ has no
conflicts in it at all (and hence is a valid $\Sigma-$structure) and
such that $M_2' \models \varphi(\tbf{a})$. We thus note that $M_2'$
has been obtained by simply resolving all the conflict cases in $M_3$
and retaining the truth values of all predicates for all their
arguments for which there is no conflict.

\end{enumerate}


\underline{\tbf{Completing the proof}}\\

With a last remaining argument now, we show that with this $M_2'$,
satisfies the last condition of the $\mathbf{EBS}$ definition.

For the proof to complete we need to show that $M_2'|_{\sigma} =
M_2|_{\sigma}$ (recall that $M_2$ is the substructure of $M$ generated
by $\mc{U}_{M_2}$). Since $\sigma$ can contain only nullary, unary,
free and existential predicates, we will consider each of these
separately.
\begin{enumerate}
\item Nullary predicates: From case (1) of \ti{Selector}, all the
  elements of $\mc{C}$ are interpreted in $M_3$, and hence in
  $M_2'$, with the same values as they are interpreted in $M$. Thus
  $M_2'|_{\mc{C}} =  M_2|_{\mc{C}}$.
\item Free and universal predicates: For a free or universal predicate
  $P$ of arity $\geq 2$, using Lemma \ref{proof-helper-1}(2),
  $\mc{P}_2$, case (3a) of $\mc{P}_1$ and the conclusion made above
  that there are no conflicts on free and universal predicates, we can
  conclude that $M_3|_{\{P\}} = M_2|_{\{P\}}$. Since in $M_2'$ is
  obtained from $M_3$ simply by fixing the conflict cases and
  retaining the truth values of all predicates for all their arguments
  for which there is no conflict, we conclude that $M_2'|_{\{P\}} =
  M_3|_{\{P\}} = M_2|_{\{P\}}$.

\item Unary predicates: For $P \in \mathsf{U}$, for the following
  cases its is easy to see that $M \models P(e)$ iff $M_3 \models
  P(e)$: (i) $P(e)$ is assigned the truth value by $\mc{P}_2$ (ii)
  $P(e) = I_{M_3}[\tbf{Z}]$ for some valuation $\tbf{Z}$ of the
  universal variables and some instance $I$ of $P$ which is free or
  universal.

  If $P(e) = I_{M_3}[\tbf{Z}]$ where $I$ is existential, then for $e
  \in \tbf{Val}(\ti{Free})$, it is easy to see from Lemma
  \ref{proof-helper-1}(1) and case (2) of $\mc{P}_1$, that $M \models
  P(e)$ iff $M_3 \models P(e)$. Else $e = a^c$ for some colour
  $c$. Then if $I_M[\tbf{Z}] = P(d_1)$, we have already seen above
  that $d_1$ and $a^c$ have the same colour $c$ in $M$. Putting this
  together with the fact from case (2) of $\mc{P}_1$ that $M \models
  I_M[\tbf{Z}]$ iff $M_3 \models I_{M_3}[\tbf{Z}]$, we have that
  $P(e)$ has the same truth value in $M$ and $M_3$. Thus in all cases
  $M \models P(e)$ iff $M_3 \models P(e)$. Since there are no
  conflicts on unary predicates, $M_3|_{\{P\}} =
  M_2|_{\{P\}}$. Further since $M_2'$ is obtained from $M_3$ simply by
  fixing the conflict cases and retaining the truth values of all
  predicates for all their arguments for which there is no conflict,
  we conclude that $M_2'|_{\{P\}} = M_3|_{\{P\}} = M_2|_{\{P\}}$.
\end{enumerate}

We conclude from the above that $M_2'|_{\sigma} = M_2|_{\sigma}$ and
indeed, that completes the proof! \epf






==> ieee_more_on_edp.tex <==
\subsection{Some observations about the $\mathbf{EDP}$
class}\label{section:obs_on_edp} 

We can see that both $\bsrS$ and $\tbf{L}_{\Sigma}$ without equality
(i.e. just the L\"owenheim class) lie wholly within $\edpSS$. In case
of $\varphi \in \bsrS$, $EV(\varphi) = \emptyset$ and hence it
contains no existential predicates at all. Hence all the conditions of
the $\edpSS$ definition are trivially satisfied.  In case of a
sentence $\varphi$ in $\tbf{L}_{\Sigma}$ without equality, it contains
no predicates of arity $\geq 2$ and no equality too. Hence all
conditions of the $\edpSS$ definition are again trivially
satisfied. Thus $\bsrS \subseteq \edpSS$ and
$\tbf{L}_{\Sigma}~\textrm{without equality}~ \subseteq \edpSS$.\\


Let for sets $A, B$ of sentences, $A \sqsubseteq B$ denote that $A$ is
semantically contained inside $B$ i.e. every sentence in $A$ is
semantically equivalent to some sentence in $B$. We then have the
following.
\begin{theorem}\label{thm:edp_lattice}
\begin{enumerate}
\item If $\sigma_1 \subseteq \sigma_2 \subseteq \Sigma$, then
$\edpS{\sigma_2} \subseteq
\edpS{\sigma_1}$.\label{thm:edp_lattice:subsumption}
\item $\edpSs = \edpS{\sigma \cup \mathsf{U}}$.
\label{thm:edp_lattice:edp_special}
\item Given $\sigma_1, \sigma_2 \subseteq \Sigma$, if $\sigma_1
\setminus \sigma_2$ contains\\ 
(a) Only unary predicates, then $\edpS{\sigma_2} \subseteq
\edpS{\sigma_1}$.\\ 
(b) A predicate of arity $\geq 2$, then $\edpS{\sigma_2}
\not\sqsubseteq \edpS{\sigma_1}$.\label{thm:edp_lattice:difference} 
\end{enumerate}
\end{theorem}

\ti{Proof}: Statements (1) and (2) above are easy to check and
statement (3)(a) follows from (1) and (2). For 3(b), let $P$ be the
arity $\geq 2$ predicate. Then consider the sentence $\phi$ as seen in
the proof of case 1 of Theorem
\ref{thm:lattice}(\ref{thm:lattice:difference}) (in section
\ref{subsection:lattice_structures}). \\

$\phi = (\bigwedge_{Q \in \Sigma \setminus \{P\}} \forall \tbf{z}_Q
Q(\tbf{z}_Q)) \wedge (\forall x \exists y P(x, y, y, \ldots, y))$

In PCNF, one can check that $\phi \in \edpS{\Sigma \setminus \{P\}}$
and hence $\phi \in \edpS{\sigma_2}$. But as shown earlier, for any
$\psi$ equivalent to $\phi$, $\psi \notin \ebsS{\sigma_1}$ and hence
by Corollary \ref{cor:edp-ebs} (in section
\ref{subsection:proof_that_edp_is_a_frag_of_ebs}), $\psi
\notin \edpS{\sigma_1}$.\epf\\


Analogous to $\mc{EBS}_{\Sigma}$, we define $\mc{EDP}_{\Sigma} =
\{\edpSs ~|~ \sigma \subseteq \Sigma\}$. Then from
Theorem \ref{thm:edp_lattice}(\ref{thm:edp_lattice:edp_special}),
$\mc{EDP}_{\Sigma} = \{\edpS{\mathsf{U} \cup \sigma} ~|~
\sigma \subseteq (\Sigma \setminus \mathsf{U})\}$. Then we have the
following.
\begin{Corollary}\label{cor:edp_lattice}
$(\mc{EDP}_{\Sigma}, \sqsubseteq)$ is a lattice which is isomorphic to
the powerset lattice $(\wp(\Sigma \setminus \mathsf{U}), \subseteq)$.
\end{Corollary}


\ti{Proof}: From Theorem
\ref{thm:edp_lattice}(\ref{thm:edp_lattice:difference}), we know that
$\edpS{\mathsf{U} \cup \sigma_1} \neq
\edpS{\mathsf{U} \cup \sigma_2}$ for $\sigma_1 \neq
\sigma_2$ where $\sigma_1, \sigma_2 \subseteq (\Sigma \setminus
\mathsf{U})$.  Consider $f:\mc{EBS}_{\Sigma} \rightarrow \wp(\Sigma \setminus
\mathsf{U})$ such that $f(\edpS{\mathsf{U} \cup \sigma}) = \Sigma
\setminus \sigma$. $f$ can be seen to be a bijection. \\

Now if $f(\edpS{\mathsf{U} \cup \sigma_1}) \subseteq
f(\edpS{\mathsf{U} \cup \sigma_2})$, then $\sigma_2
\subseteq \sigma_1$ and hence by parts
(\ref{thm:edp_lattice:subsumption}) and
(\ref{thm:edp_lattice:edp_special}) of Theorem
\ref{thm:edp_lattice}, $\edpS{\mathsf{U} \cup \sigma_1}
\subseteq \edpS{\mathsf{U} \cup \sigma_2}$. Conversely if 
$\edpS{\mathsf{U} \cup \sigma_1} \subseteq \edpS{\mathsf{U} \cup
\sigma_2}$, then since $\sigma_1$ and $\sigma_2$ cannot contain any
unary predicates, by Theorem
\ref{thm:edp_lattice}(\ref{thm:edp_lattice:difference}), it must be
that $\sigma_2 \setminus \sigma_1$ is empty. In other words,
$f(\edpS{\mathsf{U} \cup \sigma_1}) \subseteq f(\edpS{\mathsf{U} \cup
\sigma_2})$. Thus $f$ is an isomorphism from $\mc{EBS}_{\Sigma}$ to
$\wp(\Sigma \setminus \mathsf{U})$.\epf\\


The \ti{lub}($\sqcup$) and \ti{glb}($\sqcap$) operators in
($\mc{EDP}_{\Sigma}, \subseteq$) are defined as: $\edpS{\sigma_1}
\sqcup \edpS{\sigma_2} = \edpS{\sigma_1 \cap \sigma_2}$ and
$\edpS{\sigma_1} \sqcap \edpS{\sigma_2} = \edpS{\sigma_1 \cup
\sigma_2}$. Note that $\edpS{\sigma_1 \cup \sigma_2} \subseteq
(\edpS{\sigma_1} \cap \edpS{\sigma_2})$ and $ (\edpS{\sigma_1} \cup
\edpS{\sigma_2}) \subseteq \edpS{\sigma_1 \cap \sigma_2}$.\\


Finally the following result shows that except under certain
conditions, $\edpSs$ is not a syntactic characterization of $\ebsSs$
in general. Below $A \sqsubset B$ means $A \sqsubseteq B$ but $B
\not\sqsubseteq A$. Also $\cong$ means `semantic equivalence' i.e. $A
\cong B$ iff $A \sqsubseteq B$ and $B \sqsubseteq A$.

\begin{theorem}\label{theorem:comparing_edp_and_ebs}
\begin{enumerate}
\item If $\Sigma$ contains only unary predicates,
$\edpSs \cong \ebsSs \cong
\bsrS$ for all $\sigma \subseteq \Sigma$.\label{theorem:edp_unary_equals_ebs}
\item If $\Sigma$ contains a predicate of arity $\geq 2$, then \\
(a) $\edpSS \cong \ebsSS \cong
\bsrS$.\label{theorem:edp_binary_with_full_sigma_equals_ebs}\\
(b) If $\Sigma \setminus \sigma$ contains atleast one unary predicate,
then $\edpSs \sqsubset \ebsSs$.
\label{theorem:edp_binary_with_unary_not_in_sigma_is_strict_subset_of_ebs}
\end{enumerate}
\end{theorem}

\ti{Proof:} Part \ref{theorem:edp_unary_equals_ebs} above follows
from Theorem \ref{thm:lattice}(\ref{thm:lattice:collapse}) (of section
\ref{subsection:lattice_structures}) and Corollary
\ref{cor:edp-ebs} (of section
\ref{subsection:proof_that_edp_is_a_frag_of_ebs}).
Part \ref{theorem:edp_binary_with_full_sigma_equals_ebs} follows from
Theorem \ref{thm:lowest_EBS_equals_BSR} (of section
\ref{section:ebs_and_bsr}) and Corollary \ref{cor:edp-ebs}.  For part
\ref{theorem:edp_binary_with_unary_not_in_sigma_is_strict_subset_of_ebs},
let $U$ be the said unary predicate. Let $P \in \Sigma$ be a predicate
of arity $\geq 2$. Then consider the sentence $\phi$ used in the proof
of case (2) of Theorem
\ref{thm:lattice}(\ref{thm:lattice:difference}).  Now $\phi \in
\ebsSs$. But suppose it is equivalent to $\psi \in
\edpSs$. By Theorem
\ref{thm:edp_lattice}(\ref{thm:edp_lattice:edp_special}) and Corollary
\ref{cor:edp-ebs}, $\psi \in \ebsS{\sigma \cup \mathsf{U}}$. But then
from the proof of case (2) of Theorem
\ref{thm:lattice}(\ref{thm:lattice:difference}), $\psi$ cannot be in
any $\ebsS{\sigma_1}$ where $\sigma_1$ contains $\mathsf{U}$. \epf\\


We do not know whether $\ebsSs$ strictly semantically subsumes
$\edpSs$ when $\Sigma \setminus \sigma$ does not contain any unary
predicate.




\subsection{Extensions of the $\edpSs$
  class}\label{section:edp-and-other-classes}

\subsubsection{Relaxing the last condition of $\edpS{\sigma}$}

Consider the last condition in the $\edpSs$
definition disjuncted with the following condition:\\

For a predicate $P$ of arity $\geq 2$, for every pair of distinct
instances of $P$, atleast one of which is existential, either (a) the
two instances are existentially distinguishable w.r.t. $v \in
\overline{E_{\mathsf{U}}}$ or (b) the two instances are existentially
distinguishable w.r.t to every variable in $E_{1,2}$ where $E_{1, 2}$
is the set of all the $E_U$ variables appearing as arguments in the
two instances. Then the bound in this case is given by $ \mc{B} =
|V(\varphi)| + |\overline{E_{\mathsf{U}}}| + |E_{\mathsf{U}}| \cdot
2^k$.\\


\ti{Proof:}

We refer to the proof of Theorem ~\ref{thm:edp-bound} as given in
section \ref{subsection:proof_that_edp_is_a_frag_of_ebs}.  We will
need expand the initial substructure $M_1$ by making only the
following changes.  We choose $\tbf{Val}(\ti{Free})$ and
$\tbf{Val}(E_{\mathsf{U}})$ as before.  For any colour $c$, $A^c$
however is chosen as follows: Consider the set $\mc{V}_M^c$ as defined
in the proof.  Let $|E_{\mathsf{U}}| = p$. If $|\mc{V}_M^c| < p$, then
choose $A^c = \mc{V}_M^c$ (in this case we call $A^c$ to be a `small
partition'). Else let $a^c_{j_1}, \ldots, a^c_{j_p}$ be $p$ distinct
elements of $\mc{V}_M^c$ where $E_{\mathsf{U}} = \{v_{j_1}, \ldots,
v_{j_p}\}$. Then choose $A^c = \{ a^c_{j_1}, \ldots, a^c_{j_p}\}$ (in
this case we call $A^c$ as `a subset of a large partition').  As
before, let $M_1$ be the substructure generated by
$\tbf{Val}(\ti{Free}), \tbf{Val}(\overline{E_{\mathsf{U}}})$ and
$\bigcup_{c \in \{0, 1\}^k} A^c$. Then
\begin{eqnarray}
|U_M| & \leq & |\tbf{Val}(\ti{Free})| +
 |\tbf{Val}(\overline{E_{\mathsf{U}}})| +
\Sigma_{c \in \{0, 1\}^k} |A^c| \nonumber\\ 
& \leq & |V(\varphi)| + |\overline{E_{\mathsf{U}}}| +
|E_{\mathsf{U}}|\cdot2^k \nonumber 
\nonumber
\end{eqnarray}
so that $\mc{B} = |V(\varphi)| + |\overline{E_{\mathsf{U}}}| +
|E_{\mathsf{U}}|\cdot2^k$.\\


Let $\tbf{Z}$ be an instantiation of the universal variables. We
modify \ti{Selector} (which chooses the values to be assigned to $v_i
\in E_{\mathsf{U}}$) as follows. Let $d$ be the value from $M$ chosen
for $v_i$.
\begin{enumerate}
\item If $d \in \tbf{Val}(\ti{Free})$, this same value is chosen in
  $M_3$.
\item Else, let $c$ be the colour of $d$ in $M$. We have two suhcases
 here.\\
(a) If $d$ is from a small partition, then $d$ itself is chosen as
  the value for $v_i$\\
(b) Else $a^c_{i}$ is chosen as the value of $v_i$.
\end{enumerate}

Consider an instantiation \tbf{Z} of the universal variables.  Suppose
$P$ satisfies the condition above. Then for such a $P$, we perform the
assignment of truth values to the (instantiated) instances of $P$ in
$\psi_{M_3}[\tbf{Z}]$ as follows: for each instance $I$ of $P$ in
$\psi$, $I_{M_3}[\tbf{Z}]$ is assigned the same truth value in $M_3$
as $I_M[\tbf{Z}]$ is assigned in $M$ (This kind of assignment is only
for $P$ which satisfies the above condition. For existential
predicates $R$ of arity $\geq$ 2 which satisfy condition (3) of the
`basic' $\mathbf{EDP}$ definition, the assignment is as given in the
proof of Theorem \ref{thm:edp-bound} of section
\ref{subsection:proof_that_edp_is_a_frag_of_ebs}).\\ All that we need
to show now is that this assignment does not produce any conflicts for
$P$.\\

Suppose two instances conflicted. Let $I^t_{M_3}[\tbf{Z}_t]$ and
$I^f_{M_3}[\tbf{Z}_f]$ be the conflicting instances. Then
$I^t_{M_3}[\tbf{Z}_t] = I^f_{M_3}[\tbf{Z}_f] = P(\tbf{d})$ (say) and
w.l.o.g. assume that $M_3 \models I^t_{M_3}[\tbf{Z}_t]$ while $M_3
\models \neg I^f_{M_3}[\tbf{Z}_f]$. If $I^t$ and $I^f$ are free or
universal instances in $\psi$, then by Lemma \ref{proof-helper-1}
(appearing in the proof of Theorem \ref{thm:edp-bound}),
$I^t_{M_3}[\tbf{Z}_t] = I^t_M[\tbf{Z}_t]$ and $I^f_{M_3}[\tbf{Z}_f] =
I^f_{M}[\tbf{Z}_f]$. Further by our assignment of truth values above,
$M_3 \models I^{\alpha}_{M_3}[\tbf{Z}_\alpha] ~\textrm{iff}~ M \models
I^{\alpha}_{M}[\tbf{Z}_\alpha]$ for $\alpha \in \{t, f\}$. Then this
would produce a conflict in $M$ itself which we know is absent.\\ If
atleast one of $I^t$ or $I^f$ is existential, then we have the
following cases:

\begin{enumerate}
\item $I^t$ and $I^f$ are existentially distinguishable w.r.t. $v \in
  \overline{E_{\mathsf{U}}}$. Then in this case a conflict cannot
  occur by a similar reasoning as in the proof of Theorem
  \ref{thm:edp-bound}.
\item For each $v \in \overline{E_{\mathsf{U}}}$, the $i^{th}$
  argument of $I^t$ is $v$ iff the $i^{th}$ argument of $I^f$ is $v$
  (i.e. no $v$ existentially \ti{distinguishes} $I^t$ and $I^f$).
  Then as per the new condition, $I^t$ and $I^f$ are existentially
  distinguishable w.r.t. all variables in $E_{t, f}$ where $E_{t, f}$
  is the set of all $E_{\mathsf{U}}$ variables that appear as
  arguments in $I^t$ and $I^f$.\\ Suppose all the $E_{\mathsf{U}}$
  variables in $I^t_{M_3}[\tbf{Z}_t]$ and $I^f_{M_3}[\tbf{Z}_f]$ take
  values from a small partition. Then from case (2) of \ti{Selector}
  above, each $E_{\mathsf{U}}$ variable in $I^t$ takes on the same
  value in $I^t_{M_3}[\tbf{Z}_t]$ as in $I^t_{M}[\tbf{Z}_t]$. Likewise
  for $I^f$. If the $i^{th}$ argument of $I^t$ is $v \in
  \overline{E_{\mathsf{U}}}$, then so is the $i^{th}$ argument of
  $I^f$. Putting together these observations with the fact that
  $I^t_{M_3}[\tbf{Z}_t] = I^f_{M_3}[\tbf{Z}_f]$, we can infer that
  $I^t_{M}[\tbf{Z}_t] = I^f_{M}[\tbf{Z}_f]$. But since the truth
  values are preserved for corresponding instances in
  $\psi_M[\tbf{Z}]$ and $\psi_{M_3}[\tbf{Z}]$, we conclude that there
  must be a conflict in $M$ itself which we know is absent.\\ The case
  remaining is that there is some $E_{\mathsf{U}}$ variable $v_i$ in
  $E_{t, f}$ that takes on a value from a subset of a large domain
  i.e. $v_i$ is assigned a value of the form $a_i^c$. Suppose $v_i$
  appears as the $g^{th}$ argument of $I^t$. Then the $g^{th}$
  argument of $I^t_{M_3}[\tbf{Z}_t]$ is $a^c_i$. Now since $I^t$ and
  $I^f$ are existentially distinguishable w.r.t. $v_i$, the $g^{th}$
  argument of $I^f$ is either (a) $x \in \ti{Free}$ or (b) $v \in
  \overline{E_{\mathsf{U}}}$ or (c) $v_j \in E_{\mathsf{U}}$ where $j
  \neq i$. Then the $g^{th}$ argument of $I^f_{M_3}[\tbf{Z}_f]$ is
  either (a) a value from \tbf{Val}(\ti{Free}) or (b) a value from
  \tbf{Val}($\overline{E_{\mathsf{U}}}$) or (c) a value from a small
  partition or a value of the form $a_j^c$ (which is not equal to
  $a_i^c$ as $j \neq i$. In each of these cases, we can see that the
  $g^{th}$ argument of $I^f_{M_3}[\tbf{Z}_f]$ cannot be $a^c_i$. Then
  $I^t_{M_3}[\tbf{Z}_t]$ and $I^f_{M_3}[\tbf{Z}_f]$ do not conflict in
  the first place.
\end{enumerate}
Thus in each case we have shown that conflicts are not possible at
all.\\ Note that since the colour of the value assigned to $v_i$ in
$\psi_{M}[\tbf{Z}]$ and $\psi_{M_3}[\tbf{Z}]$ is the same, the
argument given for the unary predicates in the `Completing the proof'
section of the proof of Theorem \ref{thm:edp-bound} would still
hold.\epf

\subsubsection{Relaxing the equalities}

1. If equalities are also allowed between free and $E_{\mathsf{U}}$
variables (in addition to the ones given in the $\mathbf{EDP}$
definition), then the bound remains the same as the one given in
Theorem \ref{thm:edp-bound}).\\


\ti{Proof:}

We use the same construction as given in the proof of Theorem
\ref{thm:edp-bound} in section
\ref{subsection:proof_that_edp_is_a_frag_of_ebs} and show below that
it also handles the case of equalities mentioned above.  Consider the
case when equalities are also allowed between free and
$E_{\mathsf{U}}$ variables. Suppose the equality $x = v_i$ occurs in
some clause where $x \in \ti{Free}$ and $v_i \in E_{\mathsf{U}}$.  Now
according to our choice of the values for variable $v_i \in
E_{\mathsf{U}}$ given an instantiation \tbf{Z} of the universal
variables, if in the model $M$, it took on the value in
\tbf{Val}(\ti{Free}), then in the model $M_3$, we choose the same
value for it. Thus the equality $x = v_i$ evaluates to the same truth
value in $M_3$ as it does in $M$. If $v_i$ took on a value $d \notin
\tbf{Val}(\ti{Free})$, then $x = v_i$ would evaluate to
$\mathsf{False}$ in $M$. In $M_3$, $v_i$ would be assigned the value
$a^c$ where $c$ is the colour of $d$ in $M$. Since $a^c \in A^c$ and
$A^c \cap \tbf{Val}(\ti{Free}) = \emptyset$, $a^c \notin
\tbf{Val}(\ti{Free})$ and hence $x = v_i$ would evaluate to
$\mathsf{False}$ in $M_3$ as well. Thus in either case, we find that
the equality $x = v_i$ evaluates to the same truth value in $M_3$ as
it does in $M$. Thus the choice of $v_i$ as done by \ti{Selector}
handles the case of equalities between free and $E_{\mathsf{U}}$
variables as well.\epf\\

2. If equalities are also allowed between two $E_{\mathsf{U}}$
variables (in addition to the above equalities), then the bound is
given by $ \mc{B} = |V(\varphi)| + |\overline{E_{\mathsf{U}}}| +
|E_{\mathsf{U}}| \cdot 2^k$.\\

\ti{Proof:}


Consider the case when equalities are allowed between two
$E_{\mathsf{U}}$ variables. We will need expand the initial
substructure $M_1$ as constructed in the proof of Theorem
\ref{thm:edp-bound}, by making only the following changes. We choose
$\tbf{Val}(\ti{Free})$ and $\tbf{Val}(E_{\mathsf{U}})$ as before. For
any colour $c$, $A^c$ however is chosen as follows: Consider the set
$\mc{V}_M^c$ as defined earlier. Let $|E_{\mathsf{U}}| = p$. If
$|\mc{V}_M^c| < p$, then choose $A^c = \mc{V}_M^c$. Else let
$a^c_{j_1}, \ldots, a^c_{j_p}$ be $p$ distinct elements of
$\mc{V}_M^c$ where $E_{\mathsf{U}} = \{v_{j_1}, \ldots,
v_{j_p}\}$. Then choose $A^c = \{ a^c_{j_1}, \ldots, a^c_{j_p}\}$. As
before, let $M_1$ be the substructure generated by
$\tbf{Val}(\ti{Free}), \tbf{Val}(\overline{E_{\mathsf{U}}})$ and
$\bigcup_{c \in \{0, 1\}^k} A^c$. Then
\begin{eqnarray}
|U_M| & \leq & |\tbf{Val}(\ti{Free})| +
 |\tbf{Val}(\overline{E_{\mathsf{U}}})| +
\Sigma_{c \in \{0, 1\}^k} |A^c| \nonumber\\ 
& \leq & |V(\varphi)| + |\overline{E_{\mathsf{U}}}| +
|E_{\mathsf{U}}|\cdot2^k \nonumber 
\nonumber
\end{eqnarray}
so that $\mc{B} = |V(\varphi)| + |\overline{E_{\mathsf{U}}}| +
|E_{\mathsf{U}}|\cdot2^k$.\\


Let $\tbf{Z}$ be an instantiation of the universal variables. We
modify \ti{Selector} (which chooses the values to be assigned to $v_i
\in E_{\mathsf{U}}$) as follows. Let $d$ be the value from $M$ chosen
for $v_i$.
\begin{enumerate}
\item If $d \in \tbf{Val}(\ti{Free})$, this same value is chosen in
  $M_3$.
\item Else, let $c$ be the colour of $d$ in $M$. We have two suhcases
 here.\\
(a) If $v_i$ is assigned a value which is different from the values
  assigned to the other $v_j$'s where $v_j \in E_\mathsf{U}$, then
  choose $a^c_i$ for $v_i$ in $M_3$.\\
(b) Let $V$ be the set of all those $v_j$'s which have been assigned
  the same value as $v_i$. Then let $i^*$ be the least index appearing
  as subscript of some variable in $V$. Then choose $a^c_{i^*}$ for
  $v_i$ in $M_3$.
\end{enumerate}

We will now show that by the choices made as above, the new kinds of
equalities in $\psi_{M_3}[\tbf{Z}]$ will also evaluate to the same
truth value in $M_3$ as the corresponding equalities in
$\psi_M[\tbf{Z}]$ evaluate to in $M$.\\

Suppose the equality $x = v_i$ occurs in some clause where $x \in
\ti{Free}$ and $v_i \in E_{\mathsf{U}}$.  Now according to our choice
of the values for variable $v_i \in E_{\mathsf{U}}$ given an
instantiation \tbf{Z} of the universal variables, if in
$\psi_{M}[\tbf{Z}]$, it took on the value in \tbf{Val}(\ti{Free}),
then in the $\psi_{M_3}[\tbf{Z}]$ also the same value is chosen for
it. Thus the equality $x = v_i$ evaluates to the same truth value in
$M_3$ as it does in $M$. If $v_i$ took on a value $d \notin
\tbf{Val}(\ti{Free})$, then $x = v_i$ would evaluate to
$\mathsf{False}$ in $M$. In $M_3$, $v_i$ would be assigned a value in
$A^c$ which is disjoint with $\tbf{Val}(\ti{Free})$. Hence $x = v_i$
would evaluate to $\mathsf{False}$ in $M_3$ as well. Thus in either
case, we find that the equality $x = v_i$ evaluates to the same truth
value in $M_3$ as it does in $M$. \\

Suppose the equality $v_i = v_j$ occurs in some clause where $v_i, v_j
\in E_{\mathsf{U}}$. Suppose in $\psi_{M}[\tbf{Z}]$, $v_i$ and $v_j$
are assigned the same value. Then from case 2(b) of the modified
\ti{Selector} above, we know that in $\psi_{M_3}[\tbf{Z}]$ too, $v_i$
and $v_j$ would be assigned the same value. If $v_i$ and $v_j$ were
assigned different values in $\psi_{M}[\tbf{Z}]$, then they would be
assigned different values in $\psi_{M_3}[\tbf{Z}]$ as well. If not
then say $a^c_k$ is the common value assigned to both in
$\psi_{M_3}[\tbf{Z}]$. Then from case 2(b) of \ti{Selector}, it must
have been the case that $v_i$ was assigned the same value as $v_k$
(where $v_k$ is the least indexed variable in the set of all the
$E_{\mathsf{U}}$ variables whose values in $\psi_{M}[\tbf{Z}]$ were
the same as $v_i$) and also $v_j$ was assigned the same value as $v_k$
in $\psi_M[\tbf{Z}]$. Then $v_i$ and $v_j$ were assigned the same
value which contradicts the assumption made above. Thus in either case
$v_i = v_j$ evaluates to the same truth value in $M_3$ as it does in
$M$.\\

Note that since the colour of the value assigned to $v_i$ in
$\psi_{M}[\tbf{Z}]$ and $\psi_{M_3}[\tbf{Z}]$ is the same, the
argument given for the unary predicates in the `Completing the proof'
section of the proof of Theorem \ref{thm:edp-bound} would still
hold.\epf\\



\underline{\ti{Conjecture:}}\\

Generalising $\mathbf{EDP}$ with the conditions 1 and 2(b) above
together, the bound is given by\\

$\mc{B} = |V(\varphi)| + |\overline{E_{\mathsf{U}}}| +
|E_{\mathsf{U}}| \cdot 2^k$


\subsubsection{Extension to an order-sorted logic}

There has been recent work (\cite{tim_nelson}) on extending {\bsr} to
order-sorted logics. {\edpSs} being an unsorted logic which is
orthogonal to the extension presented in ~\cite{tim_nelson}, these two
extensions can be combined to yield syntactic generalizations of {\bsr}
which subsume each of the individual extensions.



\subsection{The L\"owenheim class with
  equality}\label{subsection:lowenheim-with-equality}

For the L\"owenheim class with equality, the bound $\mc{B}$ in general
is $q.2^k$ (where $q$ is the length of the quantifier
prefix)~\cite{BGG}. But this class, being a
special case of the $\edpSS$ class, from the above
results, we get the following finer bounds for the L\"owenheim class
with equality for different cases of equality.
\begin{enumerate}
\item For the L\"owenheim class extended with equality, where the
  equalities are either between (a) two free variables or (b) two
  universal variables or (c) a free and a universal variable or (d) a
  free and an $E_{\mathsf{U}}$ variable, the bound (on the size of the
  sub-model) is given by $\mc{B} = |V(\varphi)| + 2^k$.
\item For the L\"owenheim class extended with equality, if in addition to the
  above kind of equalities, equalities between $E_{\mathsf{U}}$
  variables are also allowed, then the bound is given by $ \mc{B} =
  |V(\varphi)| + |E_{\mathsf{U}}| \cdot 2^k$.
\end{enumerate}

\subsection{Complexity of the SAT problem for
  $\mathbf{EDP}$}\label{subsection:edp-sat-complexity}

The bounded model property of $\edpSs$ allows us
to also characterize the complexity of its SAT problem.
\begin{theorem}\label{thm:edp-sat-complexity}
The satisfiability problem for $\edpSs$ is
{\sc{NExpTime}}-complete.
\end{theorem}
\ti{Proof:} Indeed $\edpSs$ satisfies the two
conditions of Corollary
~\ref{corollary:nexptime_SAT_complexity_of_subclass_of_ebs} (appearing
towards the end of section
\ref{subsection:sat_problem_for_ebs_empty}): (a) The bound $\mc{B}$
for a sentence $\phi \in
\edpSs$ is $\leq 2^{O(|\phi|)}$. Then $f(\phi)$,
as defined in Lemma ~\ref{lemma:SAT_complexity_of_subclass_of_ebs} (of
section \ref{subsection:sat_problem_for_ebs_empty}), is efficiently
(polynomial time) computable and such that $f(\phi) \leq
2^{O(|\phi|)}$. (b) $\edpSs$ contains $\bsrS$ (since $\bsrS \subseteq
\edpSS \subseteq \edpSs$). \epf\\


An interesting consequence of the above result is that since the
satisfiability checking problem for both $\bsrS$ and
$\edpSs$ is {\sc{NExpTime}}-complete for all
$\sigma \subseteq \Sigma$, it means that there is an efficient
reduction from $\edpSempty$ to $\bsrS$
which yields a $\bsrS$ sentence which is equisatisfiable
with a given $\edpSempty$ sentence. There is some
recent work (~\cite{bsr-sat}) on improved heuristics in deciding
$\bsrS$ sentences. Finding an efficient reduction from
$\edpSempty$ to $\bsrS$ would
therefore help us get better heuristics to decide
$\edpSempty$ sentences as well. We present one such
reduction in Section~\ref{section:applicn}.


\section{Closure Properties of $\mc{EBS}_{\Sigma}$ and
  $\mc{EDP}_{\Sigma}$}\label{section:closure}

For $\Sigma$ which contains only unary predicates, $\ebsS{\sigma} =
\edpS{\sigma} = \FOS$. Clearly then $\ebsS{\sigma} =
\edpS{\sigma}$ are closed under $\wedge, \vee $ and $\neg$.\\
Hence below we consider $\Sigma$ to have atleast one arity $\geq 2$
predicate.

\subsection{Closure properties of $\mc{EBS}_{\Sigma}$}

Consider $\varphi_i \in \ebsS{\sigma_i}$.  Let $\mc{B}_1,
\mc{B}_2$ be the bounds for $\varphi_1, \varphi_2$ respectively.\\

1) $\wedge-$closure\\

Let $\varphi = \varphi_1 \wedge \varphi_2$. Assume $\sigma_1 =
\sigma_2 = \Sigma$.

Suppose $M \models \varphi$. Then $M \models \varphi_i$. Then there
exists a substructure $M_{i, 1}$ of $M$ such that $|\mc{U}_{M_{i, 1}}|
\leq \mc{B}_i$ which satisfies the $\ebsSS$
conditions for $\varphi_i$. Then let $M_1$ be the substructure of $M$
generated by $\mc{U}_{M_{1, 1}} \cup \mc{U}_{M_{2, 1}}$. Consider any
extension $M_2$ of $M_1$ within $M$. Since $M_2$ extends $M_{i, 1}$,
$M_2 \models \varphi_i$ (this is because $\varphi_i \in
\ebsS{\sigma_i}$). Then $M_2 \models \varphi$. Thus
$\varphi \in \ebsSS$. The bound $\mc{B}$ of
$\varphi$ is not more than $|U_{M_1}|$ which is $\leq \mc{B}_1 +
\mc{B}_2$.\\
However suppose w.l.o.g, $\sigma_1$ is not $\Sigma$. Then while
considering any common extension $M_2$ of $M_{1, 1}$ and $M_{2, 1}$
(mentioned above), to satisfy $\varphi_1$, in general, we might have
to interpret the $\Sigma \setminus \sigma_1$ predicates in a way which
might conflict with the way these predicates are interpreted in trying
to satisfy $\varphi_2$.\\

2) $\vee-$closure\\

Let $\varphi = \varphi_1 \vee \varphi_2$.

Suppose $M \models \varphi$. Then suppose $M \models \varphi_1 \wedge
\neg \varphi_2$. Then consider $M_1$ as $M_{1, 1}$ mentioned
above. Then any extension $M_2$ of $M_1$ within $M$ satisfies
$\varphi_1$ and hence $\varphi$. If $M \models \varphi_2 \wedge \neg
\varphi_1$ then consider $M_1$ as $M_{2, 1}$ mentioned above. Then any
extension $M_2$ of $M_1$ within $M$ satisfies $\varphi_2$ and hence
$\varphi$. Thus in either case $M_1$ is such that $|U_{M_1}| \leq
\tbf{max}\{\mc{B}_1, \mc{B}_2\}$. Further, the interpretations of the
$\sigma_1 \cap \sigma_2$ are guaranteed to be preserved when extending
$M_{1, 1}$ or $M_{2, 1}$. Hence $\varphi \in
\ebsS{\sigma_1 \cap \sigma_2}$. The bound for $\varphi$
is $\mc{B} = |U_{M_1}| \leq \tbf{max}\{\mc{B}_1, \mc{B}_2\}$.\\

3) $\neg-$(non)closure\\

Consider the following sentence in the vocabulary $\Sigma= \left\{
E\right\}$ where $E$ is a 2-ary predicate (If $\Sigma$ contains a
higher arity predicate, then that can simulate a 2-ary predicate and
hence we can construct an example in that case too similar to the one
shown below).
\begin{tabbing}
$\Phi$ \= $=$ \= $\forall x \neg E(x,x) \wedge \forall x \exists y
~((x \neq y) \wedge E(x,y)) \wedge$\\
\>\> $\forall x \forall y \forall z (E(x,y) \wedge E(y,z) \rightarrow
E(x,z)) $\\
 \> = \> $\forall x \forall y \forall z \exists w$\\
\>\> $(\neg E(x, x) \wedge (E(x,y) \wedge E(y,z) \rightarrow E(x,z))
\wedge$\\
\>\>$ ~(x \neq w) \wedge  E(x,w))$
\end{tabbing}
We can see that the models of this sentence are infinite DAGs. Then
$\Phi \notin \ebsSempty$. Now $\Phi$ is a
$\forall^*\exists^*$ sentence and its negation is an
$\exists^*\forall^*$ sentence which belongs to $\bsrS
\subseteq \ebsSS$.


\subsection{Closure properties of $\mc{EDP}_{\Sigma}$}

Consider $\varphi = \varphi_1 \wedge \varphi_2$ where $\varphi_i \in
\edpS{\sigma_i}$.\\

1) $\wedge-$closure\\

Let $\varphi = \varphi_1 \wedge \varphi_2$.

Let $\sigma_i^*$ be the set of all unary, free and universal
predicates appearing in $\varphi_i$. Assume $\sigma_1^* = \sigma_2^* =
\Sigma$. Then there are no existential predicates in both $\varphi_1$
and $\varphi_2$. Then in $\varphi$, firstly rename the variables of
$\varphi_2$ so that they are completely disjoint with those of
$\varphi_1$ and bring $\varphi$ in PCNF with the leftmost $\exists$
quantifiers of $\varphi$ being leftmost $\exists$ quantifiers of
$\varphi_1$ and $\varphi_2$ and the matrix of $\varphi$ being the
matrices of $\varphi_1$ and $\varphi_2$ conjuncted. Then $V(\varphi) =
V(\varphi_1) \cup V(\varphi_2)$. The predicates which were free or
universal in $\varphi_1$ or $\varphi_2$ continue to remain so in
$\varphi$ since the free or universal nature of each instance of
$\varphi_1$ or $\varphi_2$ remains unaffected upon the conjunction
since we made the variables of $\varphi_1$ and $\varphi_2$
disjoint. Thus $\mc{F} = \mc{F}_1 \cup \mc{F}_2$ and $\mc{A} =
\mc{A}_1 \cup \mc{A}_2$.  Also clearly $\mathsf{U} = \mathsf{U}_1 \cup
\mathsf{U}_2$ i.e. the unary predicates $\mathsf{U}$ of $\varphi$ are
those that appear in $\varphi_1$ (i.e. $\mathsf{U}_1$) or those that
appear in $\varphi_2$ (i.e. $\mathsf{U}_2$). Then $\Sigma = \sigma_1^*
= \sigma_2^* = \sigma_1^* \cup \sigma_2^* = \mathsf{U} \cup \mc{F}
\cup \mc{A} \subseteq \Sigma$. Since equality $\in \mc{F}_i \cup
\mc{A}_i$, we have that in $\varphi$, equality $\in \mc{F} \cup
\mc{A}$. Since there are no existential predicates in $\varphi_i$,
there are none in $\varphi$ as well. Thus $\varphi \in
\edpSS$.\\
However suppose w.l.o.g $\sigma_1^* \neq \Sigma$. Then consider the
following sentences: $\varphi_1 = \forall x \exists y P(x, y)~~,
\varphi_2 = \forall x \neg P(x, x)$. Then bringing $\varphi$ into PCNF
as explained above, we have $\varphi = \forall z \forall x \exists y
(P(x, y) \wedge \neg P(z, z))$. These two instances are not
existentially distinguishable w.r.t. $y$ - the only variable in
$\overline{E_{\mathsf{U}}}$. Then $\varphi \notin
\edpSs$ for any $\sigma \subseteq \Sigma$. (One
can construct a similar example for any other $\Sigma$ which contains
atleast one arity $\geq 2$ predicate.)\\

2) $\vee-$closure\\

Let $\varphi = \varphi_1 \vee \varphi_2$.

Assume $\sigma_1^* = \sigma_2^* = \Sigma$. Then again there are no
existential variables at all. Then by the same argument as above, it
is easy to see that $\varphi \in \edpSS$.\\
However suppose w.l.o.g $\sigma_1^* \neq \Sigma$. Then consider the
following sentences: \\

$\varphi_1 = \forall x \exists y (P(x, y) \wedge P(x, x))~;~\varphi_2
= \forall x \neg P(x, x)$. \\

Then bringing $\varphi$ into PCNF as explained above, we have $\varphi
= \forall z \forall x \exists y (P(x, y) \vee \neg P(z, z)) \wedge
(P(x, x) \wedge \neg P(z, z))$. Now $P(x, y)$ and $\neg P(z, z)$
appearing in the first and second clauses respectively differ in
polarity. But these two instances are not existentially
distinguishable w.r.t. $y$ - the only variable in
$\overline{E_{\mathsf{U}}}$. Then $\varphi \notin
\edpSs$ for any $\sigma \subseteq \Sigma$. (One
can construct a similar example for any other $\Sigma$ which contains
atleast one arity $\geq 2$ predicate.)\\

3) $\neg-$(non)closure\\

Consider $\varphi = \exists x \forall y (P(x, y) \vee \neg P(y,
y))$. Now $\varphi \in \edpSS$. But in $\neg
\varphi = \forall x \exists y (\neg P(x, y)) \wedge (P(y, y))$, the
two instances are not existentially distinguishable w.r.t. $y$ - the
only variable in $\overline{E_{\mathsf{U}}}$. Then $\varphi \notin
\edpSs$ for any $\sigma \subseteq \Sigma$. (One
can construct a similar example for any other $\Sigma$ which contains
atleast one arity $\geq 2$ predicate.)




==> intro_prelim.tex <==
\section{Introduction and Preliminaries}
 
The Bernays-Sch\"{o}nfinkel-Ramsey class (henceforth called {\bsr}) is
a widely used decidable class of first order logic
sentences~\cite{bsr-applns}.  Several recent works have addressed the
problem of efficiently checking satisfiability of {\bsr} formulae in
practice~\cite{bsr-sat}.  Motivated by the increasing interest in
{\bsr} formulae in recent times, we consider the problem of
generalizing this class both in a semantic and syntactic sense, while
retaining decidability of satisfiability checking.  In doing so, we
would like to exploit advances in decision procedures for {\bsr} to
answer corresponding questions for formulae in these more general
classes

\emph{\bfseries Preliminaries:} We represent a tuple of variables
$(x_1, x_2, \ldots x_n)$ using the shorthand {\vx}.  A first order
logic (henceforth called {\FO}) formula $\varphi(x_1, x_2, \ldots
x_n)$ with \emph{free variables} $x_1, x_2, \ldots x_n$ is represented
as $\varphi(\vx)$ for notational convenience.  A \emph{sentence} is a
formula without any free variables. The \emph{signature} or
\emph{vocabulary} of a formula is the set of all function and
predicate symbols that appear in the formula.  It is well known that
functions are ``syntactic sugar'' in first-order logic.  Specifically,
for every formula $\varphi$ with a $k$-ary function $f$, there is an
equisatisfiable formula $\psi$ with a $(k+1)$-ary predicate $P_f$,
such that the models of $\varphi$ are in one-to-one correspondence
with the models of $\psi$.  Hence, for the remainder of our
discussion, we will assume without loss of generality that the
vocabulary is relational, i.e. has only predicate symbols.  The set of
all {\FO} sentences over the vocabulary $\Sigma$ with equality as a
special interpretted predicate (the interpretation always being the
identity relation) is denoted {\FOS}.  When we talk about {\FO} over
the vocabulary $\Sigma$ without equality as a special interpretted
predicate, we will explicitly refer it to it as `{\FOS} without
equality'.  The set of all {\bsr} sentences over $\Sigma$ is denoted
{\bsrS}.  A formula $\varphi(x_1, x_2, \ldots x_n)$ is said to be in
prenex conjunctive normal form (PCNF) if it has the syntactic form
$Q_1 y_1\, Q_2 y_2\, \ldots Q_k y_k\,\, \phi(y_1, y_2, \ldots y_k,
x_1, x_2, \ldots x_n)$, where each $Q_i \in \{\forall, \exists\}$ and
$\phi(y_1, y_2, \ldots y_k, x_1, x_2, \ldots x_n)$ is a conjunction of
clauses, with each clause being a disjunction of literals, and each
literal being either an instance of a predicate or its negation.  It
is well known that every {\FO} formula is semantically equivalent to
one in PCNF.  Hence, we will focus our attention only on PCNF
formulas.  Since the satisfiability question for a {\FO} formula can
be reduced to the satisfiability of a corresponding {\FO} sentence, we
will focus only on {\FO} sentences in the sequel.

Given a relational vocabulary $\Sigma$, a \emph{$\Sigma$-structure}
$M$ consists of a \emph{universe (or domain)} of elements $\mc{U}_M$,
and an \emph{interpretation} $P^M$ of every predicate $P \in \Sigma$.
The interpretation of a $k$-ary predicate over $\mc{U}_M$ is a subset
of $(\mc{U}_M)^k$, giving all the tuples in $(\mc{U}_M)^k$ for which
$P^M$ evaluates to $\mathsf{True}$.  Given a sentence $\varphi$ over
the vocabulary $\Sigma$, a $\Sigma$-structure $M$ is said to be a
\emph{model} of $\varphi$, denoted $M \models \varphi$, if $\varphi$
evaluates to $\mathsf{True}$ when evaluated over $M$.  If $M$ is a
$\Sigma$-structure, the substructure $M'$ of $M$ generated by
$\mc{U}_{M'} \subseteq \mc{U}_M$ consists of the universe
$\mc{U}_{M'}$ and the restriction of the interpretation $P^M$ of each
predicate $P$ on $\mc{U}_{M'}$.  Given two $\Sigma$-structures $M_1$
and $M_2$ with the same universe, and a set of predicates $\sigma
\subseteq \Sigma$, we say that $M_1 \mid_\sigma = M_2 \mid_\sigma$ if
the interpretation of all predicates in $\sigma$ are the same in $M_1$
and $M_2$

Consider a {\FO} sentence $\varphi$ in PCNF.  It is well known that if
the quantifier prefix of $\varphi$ consists of only $\forall$
quantifiers (such sentences are called $\forall^*$ sentences), then
$\varphi$ is preserved in substructures.  In other words, if $M
\models \varphi$ and if $M'$ is a substructure of $M$, then $M'
\models \varphi$ as well.  The Lo\'{s}-Tarski theorem~\cite{BGG}
states that the converse also holds, i.e.  every {\FO} sentence that
is preserved in substructures is semantically equivalent to a
$\forall^*$ sentence.  Generalizing the syntactic requirements, if we
allow the quantifier prefix to be a string in $\exists^* \forall^*$,
we get a sentence in the Bernays-Sch\"{o}nfinkel-Ramsey (\bsr) class,
also called the Effectively Propositional ($\mathbf{EPR}$) class.  Let
$\mc{B}$ denote the length of the $\exists^*$ prefix of $\varphi$.  It
is not hard to see that $\varphi$ is preserved in substructures modulo
a bounded "core".  Specifically, if $M \models \varphi$, then there
exists a "core" $\mc{V}_M \subseteq \mc{U}_M$ containing at most
$\mc{B}$ elements such that every substructure $M'$ of $M$ that
contains $\mc{V}_M$ is also a model of $\varphi(\va)$.  The equivalent
of the Lo\'{s}-Tarski theorem for {\bsr} can also be obtained, and
will be discussed in Section~\ref{section:ebs_and_bsr}.

It follows from the above discussion that every $\exists^*\forall^*$
sentence has either finite or co-finite spectrum.  The converse,
however, is not true.  Indeed, there exist {\FO} sentences with
co-finite spectra that neither belong to {\bsr} nor are preserved
under substructures modulo a bounded core.  For example, consider
$\psi \equiv \forall x \exists y P(x, y)$. The spectrum of $\psi$ is
the entire set of natural numbers, and is hence co-finite.  Yet,
$\psi$ is neither in \bsr, nor is it preserved in substructures modulo
a bounded core.  A natural question to ask, therefore, is whether the
syntactic class {\bsr} or the semantic property of "preservation in
substructures modulo a bounded core" can be generalized in a natural
way to describe the set of all {\FO} sentences with finite or
co-finite spectra in the limit.  Such a generalization can be quite
useful in the study and application of fragments of {\FO} with finite
or co-finite spectra (the widely used {\bsr} class being just one of
them).  From a theoretical standpoint, this study can facilitate a
better understanding of the semantic relation between fragments of
{\FO} with finite or co-finite spectra.  It can also provide insights
into how small models of formulae belonging to certain fragments can
be constructed.  Since the satisfiability problem for every fragment
of {\FO} with finite or co-finite spectra is decidable, identifying
syntactic fragments with such spectral properties is useful in
practical applications as well.

The primary contributions of this paper are as follows.  We present a
parameterized generalization of the "preservation in substructures
modulo a bounded core" property that gives us progressively more
expressive fragments of {\FO} with finite or co-finite spectra,
culminating in the set of all {\FO} sentences with finite or co-finite
spectra in the limit.  We show that a large number of known decidable
fragments of {\FO} can be located within the fragments of this
generalization.  We also provide a parameterized syntactic
generalization of {\bsr} that gives us progressively more expressive
fragments of {\FO} starting from {\bsr}.  There has been recent work
(\cite{tim_nelson}) on extending {\bsr} to order-sorted logic. Our
syntactic generalization is an unsorted logic and is orthogonal to the
work in ~\cite{tim_nelson}.  We study the relation between this
syntactic generalisation and the parametrized semantic generalisation
mentioned above. We show that the syntactic generalization enjoys
special spectral properties that lends itself to interesting
applications like SMT solving and bounded model checking where {\bsr}
has been hitherto used.




==> lattice.tex <==
\section{Properties of the $\ebsSs$
  classes}\label{section:ebs_sigma}

The $\ebsS{\Sigma}$ property required that any model $M$ of a formula
$\phi \in \ebsS{\Sigma}$ is such that $\phi$ is also $\mathsf{True}$
in any substructure of $M$ which contains the `bounded core' of
$M$. While $\ebsS{\Sigma}$ required the preservation of the
interpretation of \ti{all} the predicates of $\Sigma$, $\ebsSs$
relaxes this requirement. It insists that the interpretation of only
the predicates of a specified subset $\sigma$ of $\Sigma$ be
preserved. The $\Sigma \setminus \sigma$ predicates are free to be
re-interpreted in any way by which $\phi$ becomes $\mathsf{True}$ in
the resulting structure. Specifically,
condition~\ref{ebs_general:cond3} in Definition \ref{def:ebs_general}
in section~\ref{section:ebs_sigma_introduction} does not require the extension
$M_2$ to satisfy $\varphi$.  Instead, it requires the existence of a
model $M_2'$ which possibly differs from $M_2$ in the interpretation
of predicates in $\Sigma \setminus \sigma$.


As an example, consider $\varphi = \forall x \exists y P(x, y)$. Here
$\Sigma = \{ P \}$. If we consider $\sigma = \emptyset$, then by
choosing $\mc{B} = 1$, for any model $M$ of size $\geq \mc{B}$, take
$M_1$ to be the substructure generated by any one element of $M$. Then
for any extension $M_2$ of $M_1$ within $M$, construct $M_2'$ by
re-interpreting $P$ to be the identity relation. Clearly then $M_2'
\models \varphi$. Thus $\varphi \in \ebsS{\emptyset}$.




If however $\sigma = \Sigma$, then consider the model $M$ in which
$\mc{U}_M = \mathbb{N}$ and $P(i, j) = \mathsf{True} ~\textrm{iff}~ j
= i+1$. Suppose $\varphi \in \ebsS{\Sigma}$. Then there exists a
sub-structure $M_1$ of $M$ of some bounded size say $\mc{B}$ such that
$M_1 \models \varphi$. Consider the highest number $i^*$ in
$\mc{U}_{M_1}$. Then there exists $j^* \in \mc{U}_{M_1}$ such that
$P(i^*, j^*)$ is $\mathsf{True}$ in $M_1$. But since $M_1 \subseteq
M$, $j^* = i^* + 1$. This contradicts the assumption that $i^*$ is the
highest number in $\mc{U}_{M_1}$. This shows that $\varphi \notin
\ebsS{\Sigma}$.\\


Let us define the family $\mc{EBS}_{\Sigma} = \{ \ebsSs | \sigma
\subseteq \Sigma \}$. In the section below, we look into set
inclusions between the different classes in $\mc{EBS}_{\Sigma}$, and
show that the poset $(\mc{EBS}_{\Sigma}, \subseteq)$ has a lattice
structure to it.


\subsection{Lattice Structure of $(\mc{EBS}_{\Sigma},
  \subseteq)$}\label{subsection:lattice_structures}



\begin{theorem}\label{thm:lattice}
\begin{enumerate}
\item If $\sigma_1 \subseteq \sigma_2 \subseteq \Sigma$, then
  $\ebsS{\sigma_2} \subseteq
  \ebsS{\sigma_1}$.
 \label{thm:lattice:subsumption}
\item If $\Sigma$ contains an arity $\geq 2$ predicate, then given
  $\sigma_1, \sigma_2 \in \Sigma$, if $\sigma_1 \setminus \sigma_2$ is
  non-empty, then $\ebsS{\sigma_2} \setminus
  \ebsS{\sigma_1}$ is also
  non-empty.\label{thm:lattice:difference}
\item If $\Sigma$ contains only unary predicates, then
  $\ebsS{\sigma_1} = \ebsS{\sigma_2}$ for
  any $\sigma_1, \sigma_2 \subseteq
  \Sigma$.\label{thm:lattice:collapse}
\end{enumerate}
\end{theorem}


\ti{Proof:}

Statement (\ref{thm:lattice:subsumption}) above is easy to
see. Consider $\phi \in \ebsS{\sigma_2}$. Then $\phi$ satisfies
condition \ref{ebs_general:cond3} of Definition \ref{def:ebs_general}
for $\sigma = \sigma_2$. Since $\sigma_1 \subseteq \sigma_2$,
$M_2'|_{\sigma_2} = M_2|_{\sigma_2}$ implies that $M_2'|_{\sigma_1} =
M_2|_{\sigma_1}$. Then $\phi$ satisfies the condition
\ref{ebs_general:cond3} for $\sigma = \sigma_1$ as well. The first
condition of Definition \ref{def:ebs_general} is independent of
$\sigma$. Then $\phi \in \ebsS{\sigma_1}$. Then $\ebsS{\sigma_2}
\subseteq \ebsS{\sigma_1}$.


We now prove statement (\ref{thm:lattice:difference}) above. We
consider the following cases.

1) $\sigma_1 \setminus \sigma_2$ contains an arity $\geq 2$
   predicate. Let $P$ be such a predicate of arity $k \geq 2$.

We use the same idea as in the example above to construct a formula
$\phi \in \ebsS{\sigma_2} \setminus
\ebsS{\sigma_1}$. Construct $\phi$ as follows.
\[
\phi = (\bigwedge_{Q \in \Sigma \setminus \{P\}} \forall \tbf{z}_Q
Q(\tbf{z}_Q)) \wedge (\forall x \exists y P(x, y, y, \ldots, y))
\] 
where $\tbf{z}_Q$ is a vector of variables where the length of the
vector is equal to the arity of $Q$. Call the first and second
conjuncts in the above formula as $\alpha$ and $\beta$
respectively. We first show that $\phi \in \ebsS{\sigma_2}$. Consider
a model $M$ of $\phi$ of size $\geq 1$. Consider any element $a \in
\mc{U}_M$ and let $M_1$ be the substructure of $M$ generated by
$\{a\}$. Consider any $M_2$ such that $M_1 \subseteq M_2 \subseteq
M$. Consider $M_2'$ obtained from $M_2$ in which the interpretation of
all the $\Sigma \setminus \{P\}$ predicates are retained as in $M_2$
(this will mean that the interpretation of the predicates of
$\sigma_2$ will also be preserved). But for $P$, since $P \notin
\sigma_2$, re-interpret $P$ to be `fully' $\mathsf{True}$, i.e. in
$M_2'$, $P$ is $\mathsf{True}$ for all values of its arguments. Now
since $\alpha$ is a $\forall^*$ formula over the vocabulary $\Sigma
\setminus \{P\}$, it is $\mathsf{True}$ in all substructures of
$M|_{\Sigma \setminus \{P\}}$. Then since $M_2'|_{\Sigma \setminus
\{P\}} \subseteq M|_{\Sigma \setminus \{P\}}$, $M_2'|_{\Sigma
\setminus \{P\}} \models \alpha$ and hence $M_2' \models
\alpha$. Further since $P$ is fully $\mathsf{True}$ in $M_2'$, $M_2'
\models \beta$. Thus $M_2' \models \phi$. This shows $\phi \in
\ebsS{\sigma_2}$ with $\mc{B} = 1$.

We now show that $\phi \notin \ebsS{\sigma_1}$. Consider the model $M$
in which $\mc{U}_M = \mathbb{N}$. Let all the predicates in $\Sigma
\setminus \{P\}$ be fully $\mathsf{True}$ in $M$. Let $P(x, y_1,
\ldots, y_{k-1}) = \mathsf{True} ~\textrm{iff} ~y_1 = y_2 = \cdots =
y_{k-1} = y ~\textrm{and} ~ y = x+1$. Consider any sub-structure $M_1$
of $M$ of size $\leq \mc{B}$ for some $\mc{B}$. Let $M_2 = M_1$ and
consider any sub-structure $M_2'$ obtained from $M_2$ by possibly
re-interpreting the predicates of $\Sigma \setminus \sigma_1$ but
keeping the interpretations of the $\sigma_1$ predicates the same. If
$M_2' \models \phi$, then $M_2' \models \beta$. Let $i^*$ be the
highest number in $\mc{U}_{M_2'} = \mc{U}_{M_2}$. Since $M_2' \models
\beta$, there exists $j^* \in \mc{U}_{M_2}$ such that $M_2' \models
P(i^*, j^*, \ldots, j^*)$. But since $P \in \sigma_1$, $M_2'|_{\{P\}}
= M|_{\{P\}}$ and hence $j^* = i^* + 1$. But that contradicts the
assumption that $i^*$ is the highest number in $\mc{U}_{M_2}$. This
shows that $\phi \notin \ebsS{\sigma_1}$.\\

2) $\sigma_1 \setminus \sigma_2$ contains only unary predicates. Then
   $P \notin \sigma_1 \setminus \sigma_2$. Let $U \in \sigma_1
   \setminus \sigma_2$. In order to save space, below $\tbf{P}(x, y)$
   is a shorthand for $P(x, y, \ldots, y)$.

Construct $\phi$ as follows.

\begin{tabular}{lll}
$\alpha_1$ & = & $\forall x \forall y_1 \ldots \forall y_{k-1} (P(x,
y_1, \ldots, y_{k-1}) \rightarrow$\\ 
& & $((y_1 = y_2) \wedge \ldots \wedge
(y_{k-2} = y_{k-1})))$ \\
$\alpha_2$& = & $\forall x \forall y ((x = y) \vee (\tbf{P}(x, y) \oplus
\tbf{P}(y, x)))~~ \wedge$\\ 
& & $\forall x \forall y \forall z (\tbf{P}(x, y) \wedge \tbf{P}(y,
z)) \rightarrow \tbf{P}(x, z)$\\
$\beta$ & = & $(\bigwedge_{Q \in \Sigma \setminus \{P, U\}} \forall
\tbf{z}_Q Q(\tbf{z}_Q))$\\
\end{tabular}
\begin{tabular}{ll}
$\textrm{succ}(x, y)$  = & $(x \neq y) \wedge \tbf{P}(x, y)
\wedge$\\
&  $\forall z ((z \neq x \wedge z \neq y \wedge \tbf{P}(x, z))
\rightarrow \tbf{P}(y, z))$\\
\end{tabular}
\begin{tabular}{lll}
$\gamma$ & = & $\forall x \forall y (succ(x, y) \rightarrow (U(x)
\leftrightarrow \neg U(y)))$\\
$\phi $ & = & $\alpha_1 \wedge \alpha_2 \wedge \beta \wedge \gamma$
\end{tabular}

Above $\oplus$ means XOR. The condition $\alpha_1 \wedge \alpha_2$
states that $P$ is essentially a linear order. $\gamma$ states that
the elements of the linear order are alternately labelled with $U$ and
$\neg U$.

We first show that $\phi \in \ebsS{\sigma_2}$. Consider any model $M$
of $\phi$ of size $\geq 1$. Let $a \in \mc{U}_M$. Then consider the
substructure $M_1$ generated by $\{a\}$. Consider $M_2$ such that $M_1
\subseteq M_2 \subseteq M$. Consider $M_2'$ obtained from $M_2$ by
interpreting all the predicates of $\Sigma \setminus \{U\}$ as in
$M_2$ but in which $U$ is interpreted such that the elements of the
linear order defined by $P$ in $M_2'$ are alternately labelled with
$U$ and $\neg U$ (the linear order amongst the elements of
$\mc{U}_{M_2'}$ is the same in $M_2'$ as the linear order amongst them
in $M$). Clearly then $M_2' \models \gamma$. Now since $\alpha_1
\wedge \alpha_2 \wedge \beta$ is a $\forall^*$ sentence over $\Sigma
\setminus \{U\}$ and since $M_2'|_{\Sigma \setminus \{U\}} \subseteq
M|_{\Sigma \setminus \{U\}}$, we have $M_2'|_{\Sigma \setminus \{U\}}
\models (\alpha_1 \wedge \alpha_2 \wedge \beta)$ and hence $M_2'
\models (\alpha_1 \wedge \alpha_2 \wedge \beta)$. Thus $M_2' \models
\phi$. This shows that $\phi \in \ebsS{\sigma_2}$ with $\mc{B} = 1$.

We now show that $\phi \notin \ebsS{\sigma_1}$. Consider a model $M$
of $\phi$ in which $\mc{U}_{M} = \mathbb{N}$, all predicates in
$\Sigma \setminus \{P, U\}$ are fully $\mathsf{True}$, $P$ is
essentially the usual '$<$' linear order and the elements of
$\mc{U}_M$ are alternately labelled with $U$ and $\neg U$.  Now
consider any sub-structure $M_1$ of $M$ of size $\leq \mc{B}$ for some
$\mc{B}$. Let the number of `$\neg U$' elements in $\mc{U}_{M_1}$ be
$m$. Then consider any subset $~\mc{U}^* \subseteq \mc{U}_M$ such that
(i) $\mc{U}_{M_1} \subsetneq \mc{U}^*$ and $\mc{U}^* \setminus
\mc{U}_{M_1}$ contains only those elements from $\mc{U}_M$ which
are labelled with a `$U$' in $M$ and (ii) if the number of `$U$'
elements of $M$ in $\mc{U}^*$ is $n$, then $n - m \geq 2$.  Let $M_2$
be the substructure of $M$ generated by $\mc{U}^*$. Then $M_1
\subseteq M_2 \subseteq M$. Now consider any sub-structure $M_2'$
obtained from $M_2$ by possibly re-interpreting the predicates of
$\Sigma \setminus \sigma_1$ but keeping the interpretations of the
$\sigma_1$ predicates the same. If $M_2' \models \phi$, then $M_2'
\models (\alpha_1 \wedge \alpha_2 \wedge \gamma)$. Then $P$ would
impose a linear order on the elements of $\mc{U}_{M_2'}$ (This linear
order would be the same as that imposed on $\mc{U}_{M_2'}$ by the
interpretation of $P$ in $M$ if $P \in \sigma_1$ and could be
different from that imposed on $\mc{U}_{M_2'}$ by the interpretation
of $P$ in $M$ if $P \notin \sigma_1$. But in either case, it would be
a linear order).  Now since $U \in \sigma_1$, the interpretation of
$U$ is the same in $M$ and $M_2'$ and hence the number of elements
labelled by $U$ and $\neg U$ in $M_2'$ are $n$ and $m$
respectively. Since $M_2' \models \gamma$, the elements of
$\mc{U}_{M_2'}$ are alternately labelled by $U$ and $\neg U$ so that
$|n - m| \leq 1$. But this contradicts the fact that $n - m \geq
2$. This shows that $\phi \notin \ebsS{\sigma_1}$.


Thus in all cases we have shown that $\ebsS{\sigma_2} \setminus
\ebsS{\sigma_1}$ is non-empty.


The proof of statement \ref{thm:lattice:collapse} of theorem
\ref{thm:lattice} is easy to see. If $\Sigma$ contains only unary
predicates, then $\FOS = \tbf{L}_{\Sigma}$. Then as seen from the
consequences of Theorem \ref{thm:lowest_EBS_equals_BSR} in section
\ref{section:ebs_and_bsr}, $\FOS \subseteq \ebsS{\Sigma}$. Then for
any $\sigma \subseteq \Sigma$, since $\ebsSs \subseteq \FOS$, we have
$\ebsSs \subseteq \ebsS{\Sigma}$. But from statement
\ref{thm:lattice:subsumption} of theorem \ref{thm:lattice}, we have
$\ebsS{\Sigma} \subseteq \ebsSs$. Thus $\ebsSs = \ebsS{\Sigma}$ for
any $\sigma \subseteq \Sigma$. \epf


 

\begin{Corollary}\label{cor:lattice}
If $\Sigma$ contains a predicate of arity $\geq 2$, then
$(\mc{EBS}_{\Sigma}, \subseteq)$ is a complete distributive lattice
which is isomorphic to the powerset lattice $(\wp({\Sigma}),
\subseteq)$. If $\Sigma$ contains only unary predicates, then
$(\mc{EBS}_{\Sigma}, \subseteq)$ collapses to the singleton lattice.
\end{Corollary}


\ti{Proof:}

Suppose $\Sigma$ contains an arity $\geq 2$ predicate. Consider
$(\mc{EBS}_{\Sigma}, \subseteq)$. Now if $\sigma_1 \neq \sigma_2$,
then from statement \ref{thm:lattice:difference} of Theorem
\ref{thm:lattice}, $\ebsS{\sigma_1} \neq \ebsS{\sigma_2}$. Then we can
define the function $f: \mc{EBS}_{\Sigma} \rightarrow \wp({\Sigma})$
given by $f( \ebsSs) = \Sigma \setminus \sigma$. If
$f(\ebsS{\sigma_1}) = f(\ebsS{\sigma_2})$ then $ \Sigma \setminus
\sigma_1 = \Sigma \setminus \sigma_2$ or $\sigma_1 = \sigma_2$ and
hence $\ebsS{\sigma_1} = \ebsS{\sigma_2}$. Thus $f$ is injective. For
every $\sigma \in \wp({\Sigma})$, $f(\ebsS{\Sigma \setminus \sigma}) =
\sigma$. Thus $f$ is surjective and hence bijective.

Suppose $\ebsS{\sigma_1} \subseteq \ebsS{\sigma_2}$. Then if $\sigma_2
\setminus \sigma_1 \neq \{\}$, then from statement
\ref{thm:lattice:difference} of Theorem \ref{thm:lattice},
$\ebsS{\sigma_1} \setminus \ebsS{\sigma_2} \neq \{\}$ violating the
assumption just made. Then $\sigma_2 \subseteq \sigma_1$ or $\Sigma
\setminus \sigma_1 \subseteq \Sigma \setminus \sigma_2$ or
$f(\ebsS{\sigma_1}) \subseteq f(\ebsS{\sigma_2})$.

Suppose $f(\ebsS{\sigma_1}) \subseteq f(\ebsS{\sigma_2})$. Then
$\Sigma \setminus \sigma_1 \subseteq \Sigma \setminus \sigma_2$ or
$\sigma_2 \subseteq \sigma_1$.  Then from statement
\ref{thm:lattice:subsumption} of Theorem \ref{thm:lattice},
$\ebsS{\sigma_1} \subseteq \ebsS{\sigma_2}$.

Thus $\ebsS{\sigma_1} \subseteq \ebsS{\sigma_2}$ iff
$f(\ebsS{\sigma_1}) \subseteq f(\ebsS{\sigma_2})$. Thus $f$ is an
isomorphism between $(\mc{EBS}_{\Sigma}, \subseteq)$ and the powerset
lattice $(\wp({\Sigma}), \subseteq)$.

Suppose $\Sigma$ contains only unary predicates. Then from Theorem
\ref{thm:lattice} (\ref{thm:lattice:collapse}), we see that
$\mc{EBS}_{\Sigma}$ contains only one element, namely
$\ebsS{\Sigma}$. \epf\\



The \ti{lub}($\sqcup$) and \ti{glb}($\sqcap$) operators in
($\mc{EBS}_{\Sigma}, \subseteq$) are defined as: $\ebsS{\sigma_1}
\sqcup \ebsS{\sigma_2} = \ebsS{\sigma_1 \cap \sigma_2}$ and
$\ebsS{\sigma_1} \sqcap \ebsS{\sigma_2} = \ebsS{\sigma_1 \cup
\sigma_2}$. Note that $\ebsS{\sigma_1 \cup \sigma_2} \subseteq
(\ebsS{\sigma_1} \cap \ebsS{\sigma_2})$ and $ (\ebsS{\sigma_1} \cup
\ebsS{\sigma_2}) \subseteq \ebsS{\sigma_1 \cap \sigma_2}$.

\subsection{$\ebsSs$ and other semantic classes}
\label{subsection:ebs_sigma_and_other_semantic_classes}

Let $\mathbf{FMP}_{\Sigma}$ be the set of all {\FOS} sentences $\phi$
such that if $\phi$ has a model, it also has a finite model. Let
$\mathbf{FSMP}_{\Sigma}$ be the set of all $\FOS$ sentences $\phi$
such that for every model of $\phi$, there is a finite sub-model of
it. One can then show the following relations of these with $\ebsSs$.

\begin{lemma}\label{lemma:ebs_fmp_fsmp}
\begin{enumerate}
\item If $\Sigma$ contains only unary predicates, then
  ${\FOS} = \mathbf{FMP}_{\Sigma} = \mathbf{FSMP}_{\Sigma} =
  \ebsSs$ for all $\sigma \subseteq
  \Sigma$. \label{lemma:ebs_fmp_fsmp:unary_case:appendix} 
\item If $\Sigma$ contains an arity $\geq 2$ predicate, then  
  $\forall ~\sigma \subseteq \Sigma$,
\begin{enumerate}
\item $\ebsSs \subsetneq
  \mathbf{FMP}_{\Sigma}$\label{lemma:ebs_fmp_fsmp:ebs_and_fmp:appendix} 
\item (i) $\ebsS{\Sigma} \subsetneq \mathbf{FSMP}_{\Sigma}$
  (ii) $\ebsSs \setminus \mathbf{FSMP}_{\Sigma}$ and
  $\mathbf{FSMP}_{\Sigma} \setminus \ebsSs$ are both
  non-empty for $\sigma \neq
  \Sigma$. \label{lemma:ebs_fmp_fsmp:ebs_and_fsmp:appendix}
\end{enumerate}
\end{enumerate}
\end{lemma}

\ti{Proof}:

Consider Statement \ref{lemma:ebs_fmp_fsmp:unary_case:appendix}
above. If $\Sigma$ contains only unary predicates, then $\FOS =
\tbf{L}_{\Sigma}$ (the L\"owenheim class with equality). Then as
seen in section \ref{section:ebs_and_bsr}, $\FOS \subseteq
\ebsS{\Sigma}$. From Theorem
\ref{thm:lattice}(\ref{thm:lattice:collapse}), for all $\sigma
\subseteq \Sigma$, $\ebsS{\Sigma} = \ebsSs \subseteq \FOS$. Then
every $\FOS$ formula has the finite model, finite sub-model and the
$\ebsSs$ properties for each $\sigma \subseteq \Sigma$.


Consider the case when $\Sigma$ contains a predicate $P$ of arity
$\geq 2$. Every $\ebsSs$ sentence is either unsatisfiable or has a
finite model (of size $\mc{B}$ where $\mc{B}$ is the bound for $\phi$)
and hence has the finite model property. Thus for all $\sigma
\subseteq \Sigma$, $\ebsS{\sigma} \subseteq
\mathbf{FMP}_{\Sigma}$. But the converse is not true. Consider the
sentence $\phi$ as below.

\begin{tabular}{ll}
$\phi = $ & $\alpha_1 \wedge \alpha_2 \wedge $\\ 
& $\forall x \forall y (\textrm{succ}(x, y) \rightarrow (\tbf{P}(x, x)
\leftrightarrow \neg \tbf{P}(y, y)) \wedge $\\
& $\exists x \exists y (\textrm{first}(x) \wedge \tbf{P}(x, x) \wedge
\textrm{last}(y) \wedge \neg \tbf{P}(y, y))$
\end{tabular}
where $\alpha_1, \alpha_2$ and $\textrm{succ}(x, y)$ are as in the
proof of case (2) of statement \ref{thm:lattice:difference} of Theorem
\ref{thm:lattice}. $\textrm{first}(x)$ and $\textrm{last}(x)$ denote
that $x$ is respectively the first and last element of the linear
order. Any finite model of $\phi$ can be seen to be `essentially' a
linear order with its elements alternately coloured and not coloured
(an element $a$ is coloured iff $\tbf{P}(a, a)$ is $\mathsf{True}$),
where the first element is coloured and the last is not. Then $\phi$
has finite models of only even cardinality. Thus $\phi$ has the finite
model property. Its easy to see that $\phi$ also has the finite
sub-model property. But from Lemma \ref{lemma:ebs_empty_model_sizes}
(in the forthcoming section \ref{section:ebs_empty}), $\phi$ cannot be
in $\ebsS{\emptyset}$ and hence from Theorem
\ref{thm:lattice}(\ref{thm:lattice:subsumption}), it cannot be in
$\ebsSs$ for any $\sigma \subseteq \Sigma$.  This shows statement
\ref{lemma:ebs_fmp_fsmp:ebs_and_fmp:appendix} and the second part of
statement \ref{lemma:ebs_fmp_fsmp:ebs_and_fsmp:appendix}(ii).

Consider statement \ref{lemma:ebs_fmp_fsmp:ebs_and_fsmp:appendix}. Now
by definition, all sentences in $\ebsS{\Sigma}$ are also in
$\mathbf{FSMP}_{\Sigma}$. Then considering $\phi$ above, we get
statement \ref{lemma:ebs_fmp_fsmp:ebs_and_fsmp:appendix}(i).

Consider $\ebsSs$. If $\Sigma \setminus \sigma$ contains a predicate
$P$ of arity $\geq 2$, then consider the sentence $\phi$ as given in
the proof of part (1) of statement \ref{thm:lattice:difference} of
Theorem \ref{thm:lattice}. This sentence cannot have the finite
submodel property. If $\Sigma \setminus \sigma$ contains only unary
predicates, then consider one such unary predicate $U$. Then consider
the sentence $\phi = \phi_1 \wedge \phi_2$ where $\phi_1$ asserts that
$P$ is essentially a linear order and $\phi_2$ asserts that either
there is no last element in the model or if there is one, then it must
be labelled with $U$. Then consider an infinite linear order in which
no element is labelled with $U$. One can see that while this models
$\phi$, no finite sub-model of this can model $\phi$. But since $U$
lies outside $\sigma$, for any finite sub-model, one can change the
interpretation of $U$ and label the last element of the finite
sub-model with $U$ to make $\phi$ true in the resulting model. Hence
$\phi \in \ebsSs$.  This finally shows the first part of
\ref{lemma:ebs_fmp_fsmp:ebs_and_fsmp:appendix}(ii). \epf







==> spectrum.tex <==
\section{Characterizing the spectra of the $\ebsSs$ classes}

The \ti{spectrum} of a sentence $\phi$ is defined as the set of
cardinalities of all the finite models of $\phi$. The spectrum of
$\phi$ is thus a subset of $\mathbb{N}$. It was proved by Ramsey
~\cite{BGG} that the spectrum of any sentence in $\bsrS$ is either
finite or co-finite.  By Theorem \ref{thm:lowest_EBS_equals_BSR} (in
section \ref{section:ebs_and_bsr}), since $\bsrS$ is the syntactic
characterization of $\ebsSS$, it follows that the spectrum of any
$\ebsSS$ sentence is also finite or co-finite.

Let $\mc{F}_{\Sigma}$ be the set of all $\FOS$ sentences which
have finite or co-finite spectra. Then from above, $\ebsSS \subseteq
\mc{F}_{\Sigma}$. We now ask: how does $\ebsSs$ compare with
$\mc{F}_{\Sigma}$?

Lemma ~\ref{lemma:ebs_empty_model_sizes} (in section
\ref{subsection:obs_about_ebs_empty}) immediately shows that
$\ebsSempty = \mc{F}_{\Sigma}$.

Thus for any $\Sigma$, $\ebsSempty$ is exactly the set of all
$\FOS$ sentences which have finite or co-finite spectra.

From Theorem \ref{thm:lattice} (in section
\ref{subsection:lattice_structures}), this implies that unless $\Sigma$
contains only monadic predicates, for each non-empty $\sigma \subseteq
\Sigma$,
\[
  \ebsSs \subsetneq \mc{F}_{\Sigma}
\]
If $\Sigma$ contains only monadic predicates, we have
\[
  \ebsSS = \mc{F}_{\Sigma}
\]

This then answers the question posed above. $\mc{F}_{\Sigma}$ is
exactly $\ebsSs$ if $\Sigma$ has only monadic predicates. If $\Sigma$
contains atleast one predicate of arity $\geq 2$, then $\ebsSs$ is a
strict semantic subset of $\mc{F}_{\Sigma}$ for a non-empty $\sigma
\subseteq \Sigma$.

Let for a set $A$ of sentences, $\mc{S}(A)$ denote the set of spectra
of the sentences in $A$. We then ask the question: How do
$\mc{S}(\ebsSs)$ for different $\sigma$ compare?

We have the following lemma.

\begin{lemma}\label{lemma:bsr_empty_spectra_equals_fin_and_cofinite_spectra}
Consider a set $\mathsf{S}$ which is finite or co-finite. Then there
exists a $\bsrempty$ formula whose spectrum is
$\mathsf{S}$.
\end{lemma}

\ti{Proof}:

Suppose $\mathsf{S}$ is finite. Let $\mathsf{S} = \{k_1, \ldots,
k_n\}$. For each $k_i$, construct $\phi_i$ as follows:

\[
\phi_i = \exists x_1 \ldots \exists x_{k_i} \forall y ((\bigwedge_{j =
1}^{j = k_i} \bigwedge_{l = j+1}^{l = k_i} (x_j \neq x_l)) \wedge
\bigvee_{j = 1}^{j = k_i} (y = x_j))
\]

$\phi_i$ asserts that there are exactly $k_i$ elements in any model of
$\phi_i$.
Then the formula

\[
\phi_{\mathsf{S}} = \bigvee_{i=1}^{i=n} \phi_i
\]
has a spectrum which is exactly $\mathsf{S}$. Note that since
$\phi_{\mathsf{S}}$ is a disjunction of $\bsrempty$
sentences, $\phi_{\mathsf{S}} \in \bsrempty$.

Suppose $\mathsf{S}$ is co-finite. Then let 

$\mathsf{S} = \left\{ k_{1}, k_{2}, \ldots, k_{n} \right\}$ $\cup$
$\left\{\mc{B} + i \mid i \ge 0 \right\}$ for some $n > 0$ where
$\mc{B}$ is larger than all the $k_i$s.

For each $k_i$, we construct $\phi_i$ as shown above. We also
construct the following sentence $\phi_\mc{B}$

\[
\phi_\mc{B} = \exists x_1 \ldots \exists x_{\mc{B}} (\bigwedge_{j =
1}^{j = \mc{B}} \bigwedge_{l = j+1}^{l = \mc{B}} (x_j \neq x_l))
\]

Then the spectrum of $\phi_\mc{B}$ is exactly $\left\{\mc{B} + i \mid
i \ge 0 \right\}$. Then the formula
\[
\phi_{\mathsf{S}} = (\bigvee_{i = 1}^{i = n} \phi_i) \vee \phi_\mc{B}
\]
has spectrum which is exactly $\mathsf{S}$. Again since
$\phi_{\mathsf{S}}$ is a disjunction of $\bsrempty$
sentences, $\phi_{\mathsf{S}} \in \bsrS$.\epf\\


\begin{Corollary}\label{cor:bsr_sigma_spectra_equals_fin_and_cofinite_spectra}
Consider a set $\mathsf{S}$ which is finite or co-finite. Then for
every $\Sigma$, there exists a $\bsrS$ formula whose spectrum is
$\mathsf{S}$.
\end{Corollary}

\ti{Proof}:

By Lemma
\ref{lemma:bsr_empty_spectra_equals_fin_and_cofinite_spectra}, there
exists a $\bsrempty$ formula $\phi_{\mathsf{S}}$ whose
spectrum is $\mathsf{S}$. Then consider the formula
$\psi_{\mathsf{S}}$ given by

\[
\psi_{\mathsf{S}} = \phi_{\mathsf{S}} \wedge \bigwedge_{Q \in \Sigma}
\forall \tbf{z}_Q Q(\tbf{z}_Q)
\]

where $\tbf{z}_Q$ is a vector of variables of length equal to the
arity of $Q$. Any finite model of $\psi_{\mathsf{S}}$ is also a model
of $\phi_{\mathsf{S}}$ and hence its cardinality must be in
$\mathsf{S}$. Conversely, for any $k \in \mathsf{S}$, there is a model
of $\phi_{\mathsf{S}}$ whose cardinality is $k$. Since
$\phi_{\mathsf{S}}$ is over the empty vocabulary, this model is just a
universe of size $k$. Then this model can be expanded to a model of
$\psi_{\mathsf{S}}$ by interpreting all the predicates of $\Sigma$ as
`fully' $\mathsf{True}$.

Thus the spectrum of $\psi_{\mathsf{S}}$ is exactly
$\mathsf{S}$.\epf\\


From the above, we see that for any $\Sigma$, $\mc{S}(\bsrS)$ is
exactly the set of all finite and co-finite sets. Then since from
Theorems \ref{thm:lowest_EBS_equals_BSR} (section
\ref{section:ebs_and_bsr}) and
\ref{thm:lattice}(\ref{thm:lattice:subsumption}) (section
\ref{subsection:lattice_structures}), $\bsrS \subseteq \ebsSS \subseteq
\ebsSs \subseteq \mc{F}_{\Sigma}$, we have that $\mc{S}(\ebsSs)$ is
exactly the set of all finite and co-finite sets. Thus, for all
$\Sigma$ and all $\sigma \subseteq \Sigma$, we have a complete
characterization of the spectra of $\ebsSs$ as the set of all finite
and co-finite sets.

Further since any $\ebs{\emptyset}{\emptyset}$ sentence $\phi$ can be
easily extended to a sentence of $\ebsSs$ which has the same spectrum
as $\phi$, the $\ebs{\emptyset}{\emptyset}$ class can be seen as the
`minimum' class in the $\mathbf{EBS}$ heirarchy whose set of all
spectra is exactly the set of all finite and co-finite sets.

